BCFA: Bespoke Control Flow Analysis for CFA at Scale

Many data-driven software engineering tasks such as discovering programming patterns, mining API specifications, etc., perform source code analysis over control flow graphs (CFGs) at scale. Analyzing millions of CFGs can be expensive and performance of the analysis heavily depends on the underlying CFG traversal strategy. State-of-the-art analysis frameworks use a fixed traversal strategy. We argue that a single traversal strategy does not fit all kinds of analyses and CFGs and propose bespoke control flow analysis (BCFA). Given a control flow analysis (CFA) and a large number of CFGs, BCFA selects the most efficient traversal strategy for each CFG. BCFA extracts a set of properties of the CFA by analyzing the code of the CFA and combines it with properties of the CFG, such as branching factor and cyclicity, for selecting the optimal traversal strategy. We have implemented BCFA in Boa, and evaluated BCFA using a set of representative static analyses that mainly involve traversing CFGs and two large datasets containing 287 thousand and 162 million CFGs. Our results show that BCFA can speedup the large scale analyses by 1%-28%. Further, BCFA has low overheads; less than 0.2%, and low misprediction rate; less than 0.01%.

==> abstract.tex <==
% Background
Source code analysis at a large scale is useful for many software engineering problems,
e.g., defect prediction, programming pattern discovery, specification inference,
etc. However source code analysis at a large scale can be very expensive thus
making its use difficult.
%  Approach
This work proposes {\em hybrid traversal}, a technique for realizing 
source code analysis expressed as traversals 
over control flow graphs more efficiently. 
Our key insight is that given the code for a source code
analysis and efficiently-computable characteristics of the input graph it is possible to select
the most efficient traversal method for that (analysis, input graph) pair.
First, by analyzing the code for the source code analysis we compute its characteristics. 
Then, when applying the analysis to the input we combine analysis's characteristics with 
input graph's characteristics to arrive at the choice of the traversal method. 
This traversal method is then used to apply that source code analysis on the input graph.
% Results
We evaluate hybrid traversal using 21 source code analyses, which are typically used as 
components of larger software engineering tasks, and two datasets consisting of
287K and 161,523K graphs respectively. 
Our evaluation shows that the overhead of hybrid traversal is between 0.01\%-0.2\%, and  
it leads to between 1\%-28\% reduction in analysis time. 
The misprediction rate for hybrid traversal is very low (<0.01\%).
The case studies show that hybrid traversal reduces 80--175 minutes in running times for three software engineering tasks.
%We also implemented 3 software engineering case studies and hybrid traversal leads to a saving of 
%between 80-175 minutes for our case studies. 
%Our newfound ability to analyze source code in massive software
%repositories such as GitHub has led to an uptick in data-driven
%solutions to software engineering problems. Source code analysis is
%often realized as traversals over source code artifacts represented as
%graphs. Since the number of artifacts that are analyzed is huge, in
%millions, the efficiency of the source code analysis technique is very
%important. The performance of source code analysis techniques heavily
%depends on the order of nodes visited during the traversals: the
%traversal strategy. For instance, selecting the best traversal strategy and optimizing it for a software engineering task, that infers the temporal specification between pairs of API method calls, could reduce the running time on a large codebase from 64\% to 96\%. 
%While, there exists several choices for traversal strategy, like depth-first, post-order, reverse post-order, etc., there exists no technique to choose the most time-efficient strategy for traversals. In this paper, we show that a single traversal strategy does not fit all source code analysis scenarios. Somewhat more
%surprisingly, we demonstrate that given the source code expressing the
%analysis task (in a declarative form) one can compute static
%characteristics of the task, which together with the runtime
%characteristics of the input, can help predict the most time-efficient
%traversal strategy for that (analysis task, input) pair. We also
%demonstrate that these strategies can be realized in a manner that is
%effective in accelerating ultra-large-scale source code analysis. Our
%evaluation shows that our technique successfully selected the most
%time-efficient traversal strategy for 99.99\%-100\% of the time and
%using the selected traversal strategy and optimizing it, the running times of a
%representative collection of source code analysis in our evaluation
%were considerably reduced by 1\%-28\% (13 minutes to 72 minutes in absolute time) when compared against the best performing traversal strategy. The overhead imposed by
%collecting additional information for our approach is less than
%0.2\% of the total running time for a large dataset that contains 287K
%Control Flow Graphs (CFGs) and less than 0.01\% for an ultra-large
%dataset that contains 162M CFGs.

==> case-studies-old.tex <==
\subsection{Case Studies}
\label{sec:case-studies}
In this section, we will look at three case studies - API Precondition mining, API Usage mining, Security Vulnerabilities (SQL injections) using Tainted Object Propagation. These three case studies were implemented using our formalism for Source Code Analysis and evaluated using Hybrid and WRPO traversal strategy. We are comparing only against WRPO since it is the next best performing traversal for all the three case studies.
\subsubsection{API Precondition mining (APM)}
This case study involves mining Github repository to derive potential preconditions
for API methods \cite{nguyen2014mining}. The key idea of this work is that API's preconditions would appear frequently in an ultra-large code corpus with a large number
of API usages, while project-specific conditions will occur less
frequently. \fignref{fig:case-study-table} shows that hybrid reduces about 175 minutes (10\%) in running time when compared against WRPO on Github dataset. 
\subsubsection{API Usage mining (AUM)}
This case study analyzes the code segments and produces a list of frequent API usage patterns for developers to inspect \cite{xie2006mapo}. This case study helps developers to understand API usages and write API client code more effectively. \fignref{fig:case-study-table} shows that hybrid reduces about 80 minutes (8\%) in running time when compared against WRPO on Github dataset.
\subsubsection{Security Vulnerabilities (SQL injections) using Tainted Object Propagation (SVT)}
This case study formulated a variety of widespread vulnerabilities, in our case SQL injections, as tainted object propagation problems \cite{livshits2005finding}. It finds all vulnerabilities (SQL injections) matching the specification within the statically analyzed code. \fignref{fig:case-study-table} shows that hybrid reduces about 84 minutes (5.5\%) in running time when compared against WRPO on Github dataset.
\input{tex-figures/case-study-table}


==> choosing.tex <==
\section{Hybrid approach}
\label{sec:hybrid-approach}
Lets look at all the candidate traversal strategies before explaining and
reasoning our decision tree.

\input{figures/candidates}

\subsection{Candidate traversal strategies}
\label{sec:candidate-traversals}
\begin{itemize}
\item \textbf{\textit{Depth-first search (DFS)}} traverses a CFG by starting at
a arbitary node as root and explores as far as possible along each branch before
backtracking.\newline
\item \textbf{\textit{Post order traversal (POS)}} traverses the vertices in the
order that they were last visited by the algorithm. In CFGs that does not
contain loops, post order guarantees that a node will be visited only after
visiting its successors.
\item \textbf{\textit{Reverse post order traversal (RPS)}} is the reverse of a
postordering, i.e. a list of the vertices in the opposite order of their last
visit. In CFGs that does not contain loops, reverse post order guarantees that a
node will be visited only after visiting its predecessors.
\item \textbf{\textit{Worklist approach}} starts off with all nodes in a
worklist. Then a node is removed from the worklist and processed. If the state
changes, then its successors (for forward dataflow problems) or predecessors
(for backward dataflow problems) are added to the worklist.  Another node is
taken from the worklist if one exists and the process repeats until the list is
empty. Worklist approach visits nodes only on demand and removes redundant visit
of nodes. Worklist approach has two types.
\begin{itemize}
\item Worklist with post ordering of nodes : In this strategy,  worklist is
initialized with post ordering of nodes.
\item Worklist with reverse post ordering of nodes : In this strategy,  worklist
is initialized with reverse post ordering of nodes.
\end{itemize}
\item \textbf{\textit{Random traversal (RAN)}} traverses a CFG in random order
of its nodes.
\end{itemize}
There are two other non-standard traversal strategies mentioned below which were
created due to the property of our CFG nodes.
\begin{itemize}
\item \textbf{\textit{Traversing in the increasing order of node ids (IN-ID)}}
This traversal visits nodes in the increasing order of their node ids. We have a
property associates with the nodes in the CFG called node id. Node ids are
assigned while constructing the CFG of the program. Node ids are assigned in a
topological order. For sequential graph, traversing the graph in the increasing
order of node ids will give the flow of the program from entry point to exit
point.

\item \textbf{\textit{Traversing in the decreasing order of node ids (DC-ID)}}
This traversal visits nodes in the decreasing order of their node ids. For
sequential graph, traversing the graph in the decreasing order of node ids will
give the backward flow of the program.
\end{itemize}

% \begin{figure*}[ht!]
% \centering
% \includegraphics[width=\linewidth]{figures/tree.pdf}
%   \caption{Traversal strategy selection decision tree.}
% \label{fig:decision-tree}
% \end{figure*}
\begin{figure}[ht!]
\centering
\includegraphics[width=\linewidth]{figures/decision.png}
\caption{Traversal strategy selection decision diagram. $P_0$ to $P_{11}$ are
markings for paths.}
\label{fig:decision-diagram}
\end{figure}

Let us reason the decisions taken by the decision tree and the optimizations
performed on it.
\subsection{Reasoning of the Decision tree}
\label{sec:Decision tree explained}
First, we check if the traversal is data flow sensitive or not. We distinguish
the traversal based on this property because traversal without data flow
completes in a single traversal of the CFG, while data flow sensitive traversal
traverses the CFG multiple time till all the nodes reach fixpoint ie the ouput
of all the nodes stabilizes. Hence the decision making process differs based on
the data flow  property. Lets look at the decision tree if the traversal is data
flow sensitive.\newline
\subsubsection{Decision tree for data flow sensitive traversal}
For data flow sensitive traversal, we look at the type of the control flow in
the CFG. This property is important now because the type of control flow
determines the number of traversal needed for data flow sensitive traversal.
\paragraph{Sequential CFG} \label{sec:decision-ds-seq}
If the graph is sequential, it means the CFG has no branches or loops. When we
know this property of graph, we can see that solving the data flow equations is
straightforward. Each node has only one predecessor/successor and hence if the
nodes are ordered in such a way that it is processed only after it's predecessor
(forward traversal) or it's successor (backward traversal), then the sequential
CFG will attain fix point in single traversal.
In order to get this ordering for sequential graph, we just have to traverse the
graph in the increasing of order of the CFG node ids (IN-ID) for forward
traversal and decreasing order of node ids (dc-id) for backward traversal. This
is because node ids are assigned in topological order as they are created and
for sequential graphs with no branches or loops, traversing the graph in the
increasing order of node ids will ensure that we traverse the node's predecessor
before the node itself. Traversing the graph in the decreasing order of node ids
will ensure that we traverse the node's successors before the node itself. Hence
hybrid traversal picks IN-ID for forward traversal and DC-ID for backward
traversal approach for sequential CFG. P-1 and P-2 in figure
\ref{fig:decision-tree} are the paths that lead to these decisions.\par
\textit{Optimization on the chosen traversal} : From the knowledge that the
graph is sequential and the traversal is data flow sensitive, hybrid approach
knows that IN-ID for forward traversal and DC-ID for backward traversal, will
complete the data flow sensitive traversal in first iteration of the CFG and we
do not have to check fixpoint in the first iteration to confirm it. Hence hybrid
approach removes fixpoint checking operation.\par

Approaches like DFS, POS, RPS, RAN will take two iteration to realize that we
have reached fix point in the first traversal, which is an overhead and an
unwanted traversal. WPOS and WRPS will visit only as much nodes as needed but it
will add an overhead of creating and maintaining the worklist. Also approaches
like DFS, POS, RPS involves accessing edge informations to determine the next
node to visit while IN-ID and DC-ID already has the nodes in order and just
visits them.\par

If the CFG is not sequential, then we check if the CFG has loops.
\paragraph{CFG with branches and no loop} \label{sec:decision-ds-br}
If the CFG does not have loop, then it is a CFG with branches and no loops. When
we know this property of graph, we can see that this CFG will stabilize in
single traversal if all predecessors of the node have been processed before the
node itself(for forward traversal) or if all the successors of the node have
been processed before the node itself(for backward traversal). RPS guarantees
such ordering for forward traversal and POS guarantees such ordering for
backward traversal. Hence hybrid picks RPS for forward traversal and POS for
backward traversal. P-9 and P-10 in figure \ref{fig:decision-tree} are the paths
that lead to these decisions.\par \textit{Optimization on the chosen traversal}
: From the knowledge that the graph has only branches and the traversal is data
flow sensitive, hybrid approach knows that RPS for forward traversal and POS for
backward traversal, will complete the data flow sensitive traversal in first
iteration of the CFG and will complete the data flow sensitive traversal in
first iteration of the CFG and we do not have to check fixpoint in the first
iteration to confirm it. Hence hybrid approach removes fixpoint checking
operation.\par Approaches like DFS, RAN, IN-ID, DC-ID will take multiple
iteration to reach fix point. WPOS and WRPS has an overhead of creating and
maintaining the worklist.

\paragraph{CFG with loops}
If the CFG has loops, it may or may not have branches other than the loop. We
next determine if the traversal is loop sensitive or not.\par \textbf{Loop
insensitive} : If the traversal is insensitive to loop, then we can just ignore
the loops present in the CFG and make decision based on the structure of the
rest of the CFG. If the CFG have branches other than the loop, then hybrid picks
RPS for forward traversal and POS for backward traversal based on the
explanation in Section \ref{sec:decision-ds-br}. P-5 and P-6 in figure
\ref{fig:decision-tree} are the paths that lead to these decisions. If the CFG
does not have branches other than the loop, then hybrid picks IN-ID for forward
traversal and DC-ID for backward traversal based on the explanation in Section
\ref{sec:decision-ds-seq}. P-7 and P-8 in figure \ref{fig:decision-tree} are the
paths that lead to these decisions.\par \textbf{Loop sensitive} : If the
traversal is loop sensitive and the CFG has loops, then no ordering of nodes can
guarantee fix point convergence in single traversal. Worklist approach is the
near best here as it visits node only on demand. Hybrid approach chooses WRPS
for forward traversal and WPOS for backward traversal. P-3 and P-4 in figure
\ref{fig:decision-tree} are the paths that lead to these decisions.\par
--------------discussion needed on why worklist is near best and not the
best-----------------\par Now let us look at the decision tree if the traversal
is data flow insensitive.
\subsubsection{Decision tree for data flow insensitive traversal}
% We check if the traversal is sensitive to the traversal strategy used.
% Traversal sensitivity means the output of the traversal changes from one
% traversal strategy to another. If the traversal is sensitive to the traversal
% strategy, then hybrid cannot pick the best strategy as we may compromise on
% the soundess of the result. We did not check this property when the traversal
% is data flow sensitive. This is because, even if data flow traversal is
% traversal sensitive, we will run the traversal till the fixpoint is reached
% and hence we will end up with the correct result.\par
If the traversal is data flow insensitive, then hybrid approach picks random
traversal. This is because since there is no data flow in the traversal, the
traversal is local to the node and is not dependent on the output of other nodes
and hence the nodes could be visited in any order.\par Other approaches like
DFS, POS, RPS involves accessing edge informations to determine the next node to
visit while WPOS and WRPS has an overhead of creating the worklist. IN-ID and
DC-ID has an unwanted contraint of accessing the nodes in order, which is an
overhead.\par Let us look at the algorithms that computes the required static
and dynamic properties.
\input{static-prop}

==> decision-tree-example.tex <==
\subsubsection{An Example}
\label{subsec:example}

In this section we explain the decision tree using an example source code analysis
and a graph.
The example analysis that we choose is the {\em Post-Dominator Analysis} shown
in Listing \ref{lst:dominators} and the graph that we choose is shown in
\fignref{fig:running-example}.
The \textit{Post-Dominator Analysis} contains two traversals: \lstinline|initT|
and \lstinline|domT|. 
The \lstinline|initT| traversal is data-flow insensitive 
%($P_{DataFlow}$ is \textit{false}) 
and loop insensitive. 
%($P_{Loop}$ is \textit{false}). 
The \lstinline|domT| traversal is data-flow sensitive 
%($P_{DataFlow}$ is \textit{true}) 
and loop insensitive. 
%($P_{Loop}$ is \textit{false}). 
The traversal directions of \lstinline|initT| and \lstinline|domT| are
\lstinline|ITERATIVE| and \lstinline|BACKWARD|, respectively. 
Our example graph in \fignref{fig:running-example} has branches and loops. 
%meaning the graph has nodes with more than one successor or
%predecessor and has cycles.
% 
% 
% For \lstinline|initT| traversal, $P_{DataFlow}$ is
% \textit{false} and $P_{Loop}$ is \textit{false}, and for \lstinline|domT|
% traversal, $P_{DataFlow}$ is \textit{true} and $P_{Loop}$ is \textit{false}. The
% traversal directions of \lstinline|initT| and \lstinline|domT| traversals are
% \lstinline|ITERATIVE| and \lstinline|BACKWARD| respectively. The connectivity of
% input graphs can be anything in the set \{sequential, branch only, loop w/o
% branch, loop w/ branch\}. We now select an optimal traversal strategy for each
% of them.

For selecting the best traversal strategies for \lstinline|initT| and the graph
with branches and loops, we fisrt check the data-flow sensitivity property of the
traversal.
As \lstinline|initT| is data-flow insensitive, \textit{ANY} traversal strategy
is picked as shown by the path $P_{11}$ in \fignref{fig:decision-diagram} and no
further checks are needed. The traversal strategy \textit{ANY} represents
nodes visited in any order.

For selecting the best traversal strategies for \lstinline|domT| and the graph
with branches and loops, we first check the data-flow sensitivity property of the
traversal.
As \lstinline|domT| is data-flow sensitive, the next property to be checked is
the graph \graphprop{}. As our input graph has loops, the next property to be
checked is whether \lstinline|domT| is loop sensitive. 
Since \lstinline|domT| is loop-insensitive, we ignore the
loops present in the graph and investigate the rest of the graph structure. As
our graph contains branches, the next property to be checked is the traversal
direction. The traversal direction for \lstinline|domT| is \lstinline|BACKWARD|,
we pick \textit{PO} traversal strategy for \lstinline|domT| traversal, as shown
by the path $P_6$ in \fignref{fig:decision-diagram}. The traversal strategy
post-order (\textit{PO}) visits all successors of a node before visiting that
node. This is most suitable for backward analysis like \lstinline|domT|, because
backward analysis analyzes successors of a node prior to analyzing the node.


==> discussions.tex <==
\subsection{Discussions}
\label{subsec:discuss}
In this section, we discuss the importance and impact of our approach for
performing analysis at large scale, and the context in which our approach is
most beneficial or not beneficial.

The poor selection of the traversal strategy could make an analysis infeasible
when performed at scale. Consider application~\cite{preconditions} that uses
analysis PDOM and RD (\fignref{tab:reduction-analyses}). For PDOM on Github
dataset, if a poor strategy is selected (e.g. RPO, WRPO), the analysis would
never finish. Similarly, for RD, a poor strategy (WPO on Github) would be ~80\%
slower. \fignref{tab:reduction-analyses} shows several `-` for Github column,
indicating that picking a poor strategy makes the analysis infeasible.

Further, several real world source code mining applications require method-level
analysis on large datasets, e.g.
\cite{preconditions,xie2006mapo,livshits2005finding}. Consider API
precondition mining~\cite{preconditions} that took ~18 hours to complete on a
single machine on SF.net dataset with 3,413 projects (4,735,151 CFGs). Such an
analysis would take ~26 days on our Github dataset (~162M CFGs), making it
impractical. Running \cite{preconditions} on a parallel infrastructure (10
machines, ~150 cores) and mining a single API (java.lang.String) took ~28 hours
on our Github dataset. Our technique was able to save 3 hours (10\%). A save of
3 hours on a parallel infrastructure is significant. If the underlying parallel
infrastructure is open/free/shared (\cite{dyer2013boa,Bajracharya-etal-04}), a 3
hour save enables supporting more concurrent users and analyses.
If the infrastructure is a paid cluster (e.g.AWS), a 3 hour less computing time
could translate to save of substantial dollar amount.




==> figures/candidates.tex <==
\begin{table}[ht!]
\centering
\caption{Candidate traversal strategies}
\label{tab:candidates}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|l}
\hline
\rowcolor[HTML]{C0C0C0} 
\textbf{\#} & \textbf{Acronym} & \textbf{Traversal Strategy}     & \textbf{Description}                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
1           & ANY              & Any order                       & Nodes can be visited in any order (random)                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
2           & INC              & Increasing order of node ids    & \begin{tabular}[c]{@{}l@{}}Nodes are visited in the increasing order of node ids\\ Node ids are assigned during the CFG construction based on the control flow order\end{tabular}                                                                                                                                                                                                                                                                             \\ \hline
3           & DEC              & Decreasing order of node ids    & Nodes are visited in the decreasing order of node ids                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
4           & PO               & Postorder                       & Successors of a node is visited before visiting the node                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
5           & RPO              & Reverse postorder               & Predecessors of a node is visited before visiting the node                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
6           & WPO              & Worklist with postorder         & \begin{tabular}[c]{@{}l@{}}Nodes are visited in the order they appear in the worklist\\ Worklist is a datastructure used to keep track of the nodes to be visited\\ Worklist is initialized with postordering of the nodes\\ Whenever a node from the worklist is removed and visited, all its \\ successors (for FORWARD) and predecessors (for BACKWARD) are\\ added to the worklist as described in ~\cite{atkinson2001implementation}\end{tabular} \\ \hline
7           & WRPO             & Worklist with reverse postorder & \begin{tabular}[c]{@{}l@{}}Similar to WPO, except that the worklist is initialized \\ with reverse postordering of the nodes\end{tabular}                                                                                                                                                                                                                                                                                                                     \\ \hline
\end{tabular}
}
\end{table}

% \begin{table}[ht!]
% \caption{Traversal strategies}
% \label{tab:strategies}
% \begin{tabular}{c|c}
% Traversal stategy & Description \\\hline\hline
% \textit{SEQ} & Sequential order \\\hline
% \textit{INC} & Increasing order of node ids \\\hline
% \textit{DEC} & Decreasing order of node ids \\\hline 
% \textit{PO} & Post order \\\hline
% \textit{RPO} & Reverse post order \\\hline 
% \textit{WPO} & Worklist with post order \\\hline
% \textit{WRPO} & Worklist with reverse post order \\\hline
% \end{tabular}
% \end{table}

==> figures/datatypes-old.tex <==
\begin{table} \centering \small
\caption{Operations on collections.}
\label{tab:operations}
% \resizebox{\textwidth}{!}{
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{|l|l|}
\hline 
\textbf{Operation} & \textbf{Description}\\\hline
\lstinline|add(C, e)| & Adding an element e to collection C \\\hline
\lstinline|addAll(C1, C2)| & Adding all elements from collection C2 to collection
C1\\\hline 
\lstinline|remove(C, e)| & Removing an element e from collection C \\\hline 
\lstinline|removeAll(C1, C2)| & Removing all elements from collection C1 that are
also present in collection C2\\\hline 
\lstinline|get(C, i)| & Element at index i from collection C is accessed\\\hline
\lstinline|has(C, e)| & Checking if collection C has element e\\\hline
\lstinline|equals(C1, C2)| & Checking if collection C1 and collection C2 has the
same elements\\\hline 
\lstinline|C1 = C2| & Assigning collection C2 to collection C1\\\hline
\lstinline|union(C1, C2)| & Returns the union of the elements in collection C1 and
collection C2\\\hline 
\lstinline|intersection(C1, C2)| & Returns the intersection of the elements in collection C1 and collection C2\\\hline
\end{tabular}
}
% }
\end{table}

==> figures/datatypes.tex <==
\begin{table} \centering \small
\caption{Operations on collections.}
\label{tab:operations}
% \resizebox{\textwidth}{!}{
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{|l|l|}
\hline 
\textbf{Operation} & \textbf{Description}\\\hline
\lstinline|add(C1, e)/addAll(C1, C2)| & Adding (an element e/all elements from collection C2) to collection C1 \\\hline
\lstinline|remove(C1, e)/removeAll(C1, C2)| & Removing (an element e/all elements present in collection C2) from collection C1 \\\hline 
\lstinline|union(C1, C2)/intersection(C1, C2)| & Returns the (union/intersection) of the elements in collection C1 and
collection C2\\\hline 
\end{tabular}
}
% }
\end{table}

==> introduction-old.tex <==
\section{Introduction}
\label{sec:introduction}

The availability of open source repositories like GitHub is driving
data-driven solutions to software engineering problems, e.g.
specification inference~\cite{preconditions}, discovering programming
patterns~\cite{taoxie-ase09}, suggesting bug
fixes~\cite{dynamine05,cpminer}, etc.
These software engineering tasks analyze different source code
representations, such as text, abstract syntax trees (ASTs), control
flow graphs (CFGs), at massive scale.
The performance of source code analysis over graphs heavily depends on
the order of the nodes visited during the traversals: {\em the
traversal strategy}. While graph traversal is a well-studied problem,
and various traversal strategies exists; e.g., depth-first,
post-order, reverse post-order, etc, no single strategy works best for
different kinds of analyses and different kinds of graphs.
Our contribution is {\em hybrid traversal selection}, a
novel source code analysis optimization technique for source code
analyses expressed as graph traversals.

\begin{figure}[t]
\centering
\subfloat[Reaching definition analysis.] {
\includegraphics[width=.32\linewidth]{figures/motivation-a-rd}
}
\subfloat[Post-dominator analysis.] {
\includegraphics[width=.32\linewidth]{figures/motivation-a-pdom}
}
\subfloat[Collector analysis.] {
\includegraphics[width=.32\linewidth]{figures/motivation-a-col}
}
\caption{Running times (ms) of the three analyses on graph A using different traversal strategies.}
\label{fig:example-a-graph}
\end{figure}

{\bf Motivation and Key Observations.\ }
To motivate, consider a software engineering task that infers the temporal 
specifications between pairs of API method calls, i.e., a call to $a$ must be 
followed by a call to $b$~\cite{engler-sosp2001,ramanathan-icse2007,weimer-tacas2005,yang-icse2006}. 
A data-driven approach for inference is to look for pairs of API calls that frequently go in pairs in 
the same order at API call sites in the client methods' code. Such an 
approach contains (at least) three source code analyses on the control flow graph 
(CFG) of each client method: 
%
1) identifying references of the API classes and call sites of the API 
methods which can be done using \emph{reaching definition} analysis~\cite{programanalysis}; 
%
2) identifying the pairs of API calls ($a$, $b$) where $b$ follows $a$ in the 
client code which can be done using \emph{post-dominator} analysis~\cite{compilers}; and 
%
3) collecting pairs of temporal API calls by traversing all nodes in the 
CFG--let us call this \emph{collector} analysis. 
%
These analyses need to be run on a large number of client methods to 
produce temporal specifications with high confidence.

Implementing each of these analyses involves traversing the CFG 
of each client method. The traversal strategy could be chosen from a 
set of standard strategies e.g depth-first search (DFS), post-order 
(PO), reverse post-order (RPO), worklist with post-ordering (WPO), 
worklist with reverse post-ordering (WRPO) and any order (ANY).

Figure \ref{fig:example-a-graph} shows the performance of each of these three 
analyses when using standard traversal strategies.
These runs are analyzing the CFG of a method in the DaCapo 
benchmark~\cite{blackburn2006dacapo}. 
Actual implementation of this method is not important, but it suffices
to know that the CFG, which we shall refer to as Graph A, has 50 nodes
and has branches but no loops. Figure \ref{fig:example-a-graph} shows
that, for graph A, the WRPO performs better than other strategies for
the reaching definition analysis while the WPO outperforms the others
for the post-dominator analysis and the ANY traversal works best for
the collector analysis.

{\bf No Traversal Strategy Fits All.\ } The performance results are
somewhat expected, but require understanding the subtleties of the
analyses. Reaching definition analysis is a forward data-flow analysis
where the output at each node in the graph is dependent on the outputs
of their predecessor nodes.
So, DFS, RPO and WRPO by nature are the most suitable.
However, worklist is the most efficient strategy here because it
visits only the nodes that are yet to reach fixpoint unlike other
strategies that also visit notes that have already reached fixpoint.
Post-dominator analysis, on the other hand, is a backward analysis
meaning that the output at each node in the graph is dependent on the
outputs of their successor nodes. Therefore, the worklist with
post-ordering is the most efficient traversal.
For the collector analysis, any order traversal works better than
other traversal strategies for graph A. This is because for this
analysis the output at each node is not dependent on the output of any
other nodes and hence it is independent of the order of nodes visited.
The any order traversal strategy does not have the overhead of
visiting the nodes in any particular order like DFS, PO, RPO nor the
overhead to maintain the worklist. Therefore any order traversal
performs better than other traversal strategies.

{\bf Properties of Input Graph Determine Strategy.\ }
For the illustrative example discussed above, DFS and RPO were worse
than WRPO for the reaching definition analysis and PO was worse than
WPO for post-dominator because they require one extra iteration of
analysis to be performed and realize that fixpoint has been reached.
However, since graph A does not have any loops, if the graph A's nodes
are visited in such a way that each node is visited after its
predecessors for reaching definition analysis and after its successors
for post-dominator analysis, then the additional iteration is actually
redundant. Given that graph A has no loops, one could optimize RPS or
PO to bypass the extra iteration and fixpoint checking. Thus, the
optimized RPS or PO would run the same number of iterations as the
respective worklist-based ones and finish faster than them because the
overhead of maintaining the list is eliminated.

\begin{figure}
\centering
\includegraphics[width=.5\textwidth]{figures/motivation-sum.pdf}
\caption{Running times of three analyses using different traversal strategies on a large codebase.}
\label{fig:motive}
\end{figure}

The potential gains of selecting a suitable traversal strategy can be 
significant.
To illustrate, consider \figref{fig:motive} that shows the performance of 
our entire illustrative example (inferring temporal specifications) on a 
large corpus of 287,000 CFGs extracted from the DaCapo
benchmark dataset~\cite{blackburn2006dacapo}.
\figref{fig:motive} shows the 
bar chart for the total running times of the three analyses. The \textbf{Best}
 strategy is an ideal one where we can always choose the most efficient with 
all necessary optimizations. The bar chart confirms that fixing a traversal 
strategies for running different analyses on different types of graphs is not 
efficient. Selecting and optimizing traversal strategy for each analysis on 
each graph is desirable. Such a strategy could reduce the running time on a 
large dataset from 64\% (against DFS) to 96\% (against RPO).

Our approach relies on our observations that a suitable traversal strategy is
dependent on both the source code analyses and input graphs' properties.
The former are static properties and the latter are runtime properties.
More importantly, depending on the properties of analyses and graphs, existing
traversals could be optimized to improve their performance.  
We have evaluated our technique using a set of 21 source code analysis that
includes control and data-flow analysis, and analysis to find bugs. The
evaluation is performed on two datasets: a dataset containing well-maintained
projects from DaCapo benchmark (contains a total of 287K graphs), and a
ultra-large dataset containing more than 380K projects from GitHub (contains a
total of 162M graphs). Our evaluation shows that our technique successfully selected
the most time-efficient traversal strategy for 99.99\%--100\% of the time and
using the selected traversal strategy and optimizing it, the running times of a
representative collection of source code analysis in our evaluation
were considerably reduced by 1\%-28\% (13 minutes to 72 minutes in absolute time) when compared against the best performing traversal strategy.
The overhead imposed by our approach is negligible (less than 0.2\% of the total 
running time for a large dataset and less than 0.01\% for an ultra-large dataset). 

In summary, this paper makes the following contributions:
\begin{itemize}
  \item It describes a system for expressing source code analysis as traversals. The
  constructs and operations in the system allows different source code analysis to
  be expressed in a manner that allows automatic selection of the best traversal
  strategies.
  \item It defines a set of novel properties about the traversal expressed 
  in our system. It also describes algorithms for analysing traversals for inferring 
  these properties. 
  \item It describes a novel decision tree for selecting the most suitable traversal 
  strategy. The static and runtime properties also allows
  certain optimizations to be performed on the selected traversal strategy to
  further improve the performance.
  \item It demonstrates the potentially broad range of applications of
  hybrid traversal selection for optimizing source code analysis such
  as available expressions, local may alias, live variable, nullness
  analysis, post-dominator, reaching definitions, resource status,
  very busy expression, etc.
\end{itemize}

==> language.tex <==
\subsection{Formalism for Source Code Analysis}
\label{sec:language}

% \subsection{Program analysis and traversals}
% \label{sec:programanalysis}
A source code analysis could be performed on various representations such as
source code text, abstract syntax trees (ASTs) or 
graph-based representations like control flow graphs (CFGs) and call
graphs (CGs). In our system, source code analysis 
are expressed as traversals over CFGs, specifically control- and
data-flow analysis.

\begin{definition}\label{def:cfg}
A control flow graph (CFG) is a directed graph $G$~=~$(N, E)$ 
with a set of nodes $N$ representing the program statements and a set
of edges $E \subseteq N \times N$ representing the control flow relation
between the program statements. 
%A CFG has a single start node, $n_{start}$, and a set of end nodes, $N_{end}$. 
\end{definition}

% A source code analysis such as control flow analysis, data-flow analysis, etc can be
% expressed as traversals over program graphs.
% \begin{definition}\label{def:cfg}
% A \textbf{Program Graph} of a program is defined as $G$ = $(N, E, n_{start},
% N_{end})$, where $G$ is a directed graph with a set of nodes $N$ representing program statements,
% and a set of edges $ E \subseteq N \times N$ representing analysis relevant
% relationship between the nodes in the graph.
% 
% representing possible flow of execution between the nodes in the
% graph.
% A program graph has a single start, $n_{start}$, and a set of end nodes, 
% $N_{end}$.
% All the nodes in a program graph are reachable from the $n_{start}$ and the
% $n_{end}$ node is reachable from all nodes in the program graph.
% \end{definition}
For any node $n \in N$, $n.preds$ is a set of immediate predecessors, $n.succs$
is a set of immediate successors, $n.stmt$ provides the program statement at the
node, and $n$.\lstinline|id| is a unique identifier of the node. Here on, we use graph to
refer to CFG.
% Note that, depending on the analysis, node ids are assigned while constructing
% the graph. For instance, in case of control flow graphs, node ids may be
% assigned in the order of the flow of execution.
% Note that, node ids are assigned in the order of the flow of
% execution, while constructing a graph. 
% Examples of program graph includes control flow graph (CFG), control dependence
% graph (CDG), program dependence graph (PDG), etc. Hereon, we refer to program
% graphs simply as graphs. 
% 
% \newline \tab $n.preds = P$ where $P =
% \{p_{0}, p_{1},.., p_{p}\}$ such that $\forall p_{i}, (p_{i}, n) \in E$,
% \newline \tab $n.succs = S$ where $S = \{s_{0}, s_{1},.., s_{s}\}$ such that
% $\forall s_{i}, (n, s_{i}) \in E$, \newline \tab $n.stmt$ = program statement
% contained in the node $n$, \newline \tab $n.id$ = unique identifier of the node
% $n$. $ids$ are integers that are assigned to the nodes in topological order.
% \end{definition}

A source code analysis over a graph visits nodes in the graph in certain order
and collects information at nodes (aka, analysis facts or outputs). For
instance, the {\em reaching definition} analysis over a CFG, visits every node
and collects the variable definitions at nodes as analysis facts.
An analysis may require multiple traversals over a graph and each traversal may
visit nodes multiple times (for fixpoint).
For instance, the {\em reaching definition} analysis requires two traversals: 
an {\em initialization} traversal for collecting the variable
definitions at nodes as analysis facts, and a {\em propagation} traversal for
propagating the analysis facts along the graph. The {\em initialization}
traversal visits every node exactly once, whereas the {\em propagation}
traversal may visit each node multiple times until a fixpoint is reached and the
analysis facts at nodes do not change further.

% A program analysis, such as control or data flow analysis visits nodes in
% the CFG, in certain order, and collects analysis facts at nodes. For
% instance, the {\em reaching definition} analysis visits every node in the CFG
% and collects variable definitions at nodes as analysis facts. An analysis
% may require multiple traversals of a CFG. For instance, the {\em reaching
% definition} analysis, in the {\em initialization} traversal, collects variable
% definitions at nodes as analysis facts, and in the {\em propagation}
% traversal, updates the analysis facts until a fixpoint is reached, where no
% further changes to analysis facts at nodes is required.

\para{An Example: Post-dominator analysis} Let us take an example source code 
analysis and describe our system to express source code analysis as traversals.
Post-dominator analysis is a backward control flow analysis that collects node
ids of all nodes that post-dominates every node in the CFG~\cite{compilers}.
This analysis can be expressed using our system as shown in Listing
\ref{lst:dominators} which mainly defines two traversals \lstinline|initT|
(lines 2-4) and \lstinline|domT| (lines 5-14). 

\begin{lstlisting}[basicstyle=\footnotesize\ttfamily, numbers=left, numbersep=-8pt, 
escapechar=@, caption={Post-dominator analysis: an example source code analysis
expressed using our system.}, label={lst:dominators}] 
		allNodes: Set<int>;
		initT := traversal(n: Node) {
			add(allNodes, n.id);
		}
		domT := traversal(n: Node): Set<int> { 
			Set<int> dom;
			if (output(n, domT) != null) dom = output(n, domT);
			else if (node.id == exitNodeId)	dom = {};
			else	dom = allNodes;
			foreach (s : n.succs) 
				dom = intersection(dom, output(s, domT)) 
			add(dom, n.id); 
			return dom; 
		} 
		fp := fixp(Set<int> curr, Set<int> prev): bool {
			if (equals(curr, prev))	return true;
			return false;
		}
		traverse(g, initT, ITERATIVE); @\label{line:traverse}@
		traverse(g, domT, BACKWARD, fp); 				
\end{lstlisting}

In our system, a source code analysis over a graph is expressed by defining and
invoking one or more traversals. A traversal is defined using a special
\lstinline|traversal| block: 
\begin{lstlisting} 
t := traversal(n : Node) : T { tbody }
\end{lstlisting}
In this traversal block definition, \lstinline|t| is the name of the traversal
that takes a single parameter \lstinline|n| representing the graph node that is
being visited. A traversal may define a return type \lstinline|T| representing
the output type. The output type can be a primitive or a collection data type. In our example, the traversal
\lstinline|initT| does not define any output for CFG nodes, whereas, the
traversal \lstinline|domT| defines an output of type \lstinline|Set<int>| for
every node in the CFG. A block of code that generates the traversal output at a graph node is given by
\lstinline|tbody|. The \lstinline|tbody| may contain common statements and
expressions, such as variable declarations, assignments, conditional statements,
loop statements, and method calls, along with some special expressions discussed
in this section.
These traversals are invoked by using a special \lstinline|traverse| expression (lines 19 and 20).
\begin{lstlisting}
traverse(g, t, d, fp)
\end{lstlisting}

A \lstinline|traverse| expression takes four parameters: \lstinline|g| is the
graph to be traversed, \lstinline|t| is the traversal to be invoked,
\lstinline|d| is the traversal direction and \lstinline|fp| is an optional 
variable name of the user-defined fixpoint function. A
traversal direction is a value from the set \{\lstinline|FORWARD|,
\lstinline|BACKWARD|, \lstinline|ITERATIVE|\}. \lstinline|FORWARD| is used
to represent a forward analysis (predecessors of a node are processed before the
node). \lstinline|BACKWARD| is used to represent a backward analysis (successors
of a node are processed before the node). \lstinline|ITERATIVE| is used to
represent a sequential analysis (visits nodes as they appear in the nodes
collection).

Lines 15-18 defines a
fixpoint function using \lstinline|fixp| block, used in the
\lstinline|traverse| expression in line 20.
%
\lstinline|fixp| is a keyword for defining a
fixpoint function. A fixpoint function can take any number of parameters, and 
must always return a boolean. A fixpoint function can be assigned a name, which
can be passed in the \lstinline|traverse| expression.

Line 1 defines a variable \lstinline|allNodes| of type 
\lstinline|Set<int>| which defines a collection type \lstinline|Set| with elements of
type \lstinline|int|. Our system provides primitive and
collection data types. Collection types include: \lstinline|Set and Seq|, where \lstinline|Set| is a
collection with unique and unordered elements, whereas, \lstinline|Seq| is a
collection with non unique but ordered elements. Important set of operations that can be
performed on collection types are \textbf{\textit{add(C1, e)}} that adds an element e to collection C1, \textbf{\textit{addAll(C1, C2)}} that adds all elements from collection C2 to collection C1, \textbf{\textit{remove(C1, e)}} that removes an element e from Collection C1, \textbf{\textit{removeAll(C1, C2)}} that removes all elements present in collection C2 from collection C1, \textbf{\textit{union(C1, C2)}} that returns union of the elements in C1 and C2 and \textbf{\textit{intersection(C1, C2)}} that returns intersection of the elements in C1 and C2. Line 3 in our example uses an operation \lstinline|add| on collection \lstinline|allNodes|.

A usage of special expression
\lstinline|output(n, domT)| can be seen in~line 7. This is used for querying the
traversal output associated with a graph node \lstinline|n|, in the traversal
\lstinline|domT|. The
traversal \lstinline|domT| defines an output of type \lstinline|Set<int>| for
every node in the CFG. For managing the analysis output of nodes,
\lstinline|domT| traversal maintains an internal map that contains analysis
output for every node, which can be queried using \lstinline|output(n, domT)|.
A pre-defined variable \lstinline|g| that represents the CFG is used in the
\lstinline|traverse| expressions in lines 19--20.

\input{tex-figures/algorithms/postdominator.tex}
\fignref{fig:running-example} takes an example graph, and shows the results of
\lstinline|initT| and \lstinline|domT| traversals. Our example graph is a CFG
containing seven nodes with a branch and a loop. The \lstinline|initT| traversal
visits nodes sequentially and adds node \lstinline|id| to the collection
\lstinline|allNodes|. The \lstinline|domT| traversal visits nodes in the
post-order\footnote{The traversal strategies chosen for \lstinline|initT| and
\lstinline|domT| traversals are explained in \secnref{sec:decision-tree}.} and
computes a set of nodes that post-dominate every visited node (as indicated by
the set of node ids). For instance, node 7 is post-dominated by itself, hence
the output at node 7 is \{7\}.
In \fignref{fig:running-example}, under \lstinline|domT| traversal, for each
node visited, we show the key intermediate steps indicated by $@$ line number.
These line numbers correspond to the line numbers shown in Listing
\ref{lst:dominators}. We will explain the intermediate results while visiting
node 2. In the \lstinline|domT| traversal, at line 9, the output set
\lstinline|dom| is initialized using \lstinline|allNodes|, hence \lstinline|dom|
= \{0, 1, 2, 3, 4, 5, 6, 7\}. At line 10, node 2 has two successors: \{3, 4\}.
At line 11, \lstinline|dom| is updated by performing an
\lstinline|intersection| operation using the outputs of successors 3 and 4. Since the
outputs of 3 and 4 are \{1, 3, 5, 6, 7\} and \{1, 4, 5, 6, 7\}, respectively, 
\lstinline|dom| set becomes
\{1, 5, 6, 7\}. At line 12, the \lstinline|id| of the visited node is added to the
\lstinline|dom| set and it becomes \{1, 2, 5, 6, 7\}.
Hence, the post-dominator set for node 2 is \{1, 2, 5, 6, 7\}. 
The post-dominator sets for other nodes are calculated similarly.

% 
% 
% \textit{Dominator analysis} written using the traversal constructs is shown in
% Figure \ref{fig:dominator}. The goal of this analysis is to find the dominator
% of each node in the cfg. Initially we have to traverse the cfg to collect all
% the nodes present in the cfg. This is realized by the init traversal in line
% which adds \textit{Dominator analysis} has two traversals - \texttt{init,
% dominator}. Line 24 applies \texttt{init} traversal on control flow graph
% \texttt{g} and the traversal direction is \texttt{FORWARD}, which means
% traversing the graph \texttt{g} from start node to end node. \texttt{init}
% traversal visits every node in the graph \texttt{g} and returns an output of
% type \texttt{int} (Line 2). Line 3 in \texttt{init} traversal has a global
% variable \texttt{allNodes} collecting the node ids. \texttt{init} traversal
% returns the current node's id as output. Line 25 applies \texttt{dominator}
% traversal on graph \texttt{g} and the traversal direction is \texttt{FORWARD}.
% It also takes fixpoint function \texttt{fp} which implies that
% \texttt{dominator} traversal will be called multiple times till the fixpoint is
% reached. Line 8 queries the output of node \texttt{n} associated with
% \texttt{dominator} traversal. If there is no output, it means that this is the
% first time node \texttt{n} is traversed using \texttt{dominator} traversal. So
% we assign \texttt{dom} to \texttt{allNodes} which contains ids of all the nodes.
% If there is output for node \texttt{n} asscoiated with \texttt{dominator}
% traversal, then we assign the output to the \texttt{dom} (Line 10-12). Line
% 13-14 merges the \texttt{dom} with the node \texttt{n}'s predecessor's output
% associated with \texttt{dominator} traversal using the \texttt{intersection}
% operation. Line 15 queries the output of node \texttt{n} associated with
% \texttt{init} traversal and assigns to \texttt{gen} variable. This also implies
% that \texttt{init} traversal should be applied before \texttt{dominator}
% traversal. Line 16-17 adds the \texttt{gen} variable to \texttt{dom} and returns
% it as output.

%\textit{Dominator analysis} written using the traversal constructs is shown in Figure \ref{fig:dominator}. \textit{Dominator analysis} has two traversals - \texttt{init, dominator}. Line 24 applies \texttt{init} traversal on control flow graph \texttt{g} and the traversal direction is \texttt{FORWARD}, which means traversing the graph \texttt{g} from start node to end node. \texttt{init} traversal visits every node in the graph \texttt{g} and returns an output of type \texttt{int} (Line 2). Line 3 in \texttt{init} traversal has a global variable \texttt{allNodes} collecting the node ids. \texttt{init} traversal returns the current node's id as output. Line 25 applies \texttt{dominator} traversal on graph \texttt{g} and the traversal direction is \texttt{FORWARD}. It also takes fixpoint function \texttt{fp} which implies that \texttt{dominator} traversal will be called multiple times till the fixpoint is reached. Line 8 queries the output of node \texttt{n} associated with \texttt{dominator} traversal. If there is no output, it means that this is the first time node \texttt{n} is traversed using \texttt{dominator} traversal. So we assign \texttt{dom} to \texttt{allNodes} which contains ids of all the nodes. If there is output for node \texttt{n} asscoiated with \texttt{dominator} traversal, then we assign the output to the \texttt{dom} (Line 10-12). Line 13-14 merges the \texttt{dom} with the node \texttt{n}'s predecessor's output associated with \texttt{dominator} traversal using the \texttt{intersection} operation. Line 15 queries the output of node \texttt{n} associated with \texttt{init} traversal and assigns to \texttt{gen} variable. This also implies that \texttt{init} traversal should be applied before \texttt{dominator} traversal. Line 16-17 adds the \texttt{gen} variable to \texttt{dom} and returns it as output.

%Live variable analysis written using the traversal constructs is shown in Figure \ref{fig:live-variable}. Line 1 denotes the node properties. Each node has a property called stmt which represents program statements. \textit{Live variable} has three traversal blocks. \textit{kill\_traversal} captures the variables that are defined in the node. In this traversal, output of each node is the variable defined in it, which we call as killed variables in this analysis. In \textit{gen\_traversal}, output of each node is the variable used in it, which we call as generated variables. The \textit{live\_analysis} traversal is the traversal which performs the live variable analysis. This traversal is called with fixpoint function as it is a data flow analysis and runs till the fixpoint is reached. The traverse method calls in line 29, 30, 31 calls the respective traversals passed.
% 
% The next section gives an overview of our approach where we analyse our
% traversal and the input cfg to arrive at the best traversal strategy to traverse
% the graph.


==> motivation-figures.tex <==
\begin{figure*}[ht!]
\begin{minipage}{\linewidth}
\centering
\includegraphics[width=0.74\linewidth]{tex-figures/grapha-motivation.png}
  \caption[Bar chart showing the execution time for dominator analysis, live variable analysis, used variable analysis using dfs traversal, post order, reverse post order traversal, worklist algorithm using post ordering of nodes, worklist algorithm using reverse post ordering of nodes and random order traversal on Graph A. Graph A has 100 nodes and has branches but no loops.]
{Bar chart showing the execution time for dominator analysis, live variable analysis, used variable analysis using dfs traversal, post order, reverse post order traversal, worklist algorithm using post ordering of nodes, worklist algorithm using reverse post ordering of nodes and random order traversal on Graph A. Graph A has 100 nodes and has branches but no loops.}
\label{fig:grapha}
\end{minipage}
\begin{minipage}{\linewidth}
\centering
\includegraphics[width=0.74\linewidth]{tex-figures/graphb-motivation.png}
  \caption[Bar chart showing the execution time for dominator analysis, live variable analysis, used variable analysis using dfs traversal, post order, reverse post order traversal, worklist algorithm using post ordering of nodes, worklist algorithm using reverse post ordering of nodes and random order traversal on Graph B. Graph A has 100 nodes and has loops.]
{Bar chart showing the execution time for dominator analysis, live variable analysis, used variable analysis using dfs traversal, post order, reverse post order traversal, worklist algorithm using post ordering of nodes, worklist algorithm using reverse post ordering of nodes and random order traversal on Graph B. Graph A has 100 nodes and has loops.}
\label{fig:graphb}
\end{minipage}

\end{figure*}



==> motivation-v2.tex <==
\section{Motivation}
\label{sec:motivation}
Lets consider three analysis - \textit{Live Variable analysis}~\cite{graham1976fast}, ~\cite{hecht1977flow}, \textit{Dominator analysis}, \textit{Used variables}. \textit{Live variable analysis} is a classic data-flow analysis performed by compilers to calculate the variables that are live at each program point. \textit{Dominator analysis} finds the dominators of each node in the graph. A node d dominates a node n if every path from the entry node to n must go through node d. \textit{Used variables analysis} finds the variables that are used at each program point.\newline
%\input{motivation-figures}
Lets run these analysis on SourceForge dataset which contains over 7 million control flow graphs using dfs, reverse postorder, posorder, worklist approach, random traversal strategies to traverse the cfgs. We recorded the time taken for the analysis to complete on each cfg using each traversal strategy and we also record the best execution time among them. The best execution time for a cfg is nothing but the lowest execution time to complete the analysis. Figure shows 8 bars indicating the total execution time of analysis on all cfgs using the traversal strategies. The first seven bars are for the seven different traversal strategies and the last bar is the sum of the execution time of the best traversal strategy. Figure shows that if we have the knowledge about the best traversal strategy for each cfg, we could save about \_\_\_ time when compared to the \_\_\_ traversal which has the best execution time when using single traversal strategy for the whole dataset for live variable analysis. We could also save about \_\_\_ time when compared to next best traversal for dominator and \_\_\_ time when compared to next best traversal for used variable analysis. This shows that for an analysis, no single traversal strategy is the best for all the cfs as we see signficant difference between the execution time of single best traversal strategy and the accumulation of best execution times. This also leads us to the intuition that the cfgs have some characteristics that warrant certain traversal strategies. \newline
But the knowledge about the characteristics of the grah alone is not enough as Figure shows that the single best traversal strategy is different across the analysis \_\_\_ has the best execution time for live variable analysis, while \_\_\_ is the best for dominator and \_\_\_ is the best for used variable analysis. This drives the point that the best traversal strategy for a cfg is different  across the analysis. This shows that for a cfg, the best traversal strategy to complete the analysis differs across the analysis. This also leads us to the intuition that the analysis have some characteristics that gives us information about the best traversal strategy for a cfg. \newline

%The above example motivates the need to identifying the best traversal strategy when we analyze large scale software repositories which contains a variety of projects with methods with different characteristics, which warrants different traversal strategy for faster analysis.

%Lets also consider two graphs A and B. These graphs are control flow graphs of methods belonging to projects in dacapo benchmark. Graph A has 100 nodes and has branches but no loops. Graph C has 100 nodes and contains loops. Let us use dfs, reverse postorder, posorder, worklist, random traversal strategies to traverse the graphs A and B and run the above mentioned analysis on these graphs and record the time taken for the analysis to complete for each traversal strategy. Figure \ref{fig:grapha} shows that for graph A, post order algorithm performs better than other traversal strategies for \textit{live variable analysis}. This is because \textit{live variable analysis} is a backward data flow analysis and the output at each nodes in the graph are dependent on the output of their successor nodes. Data flow analysis involves multiple traversals of the graph and the analysis is completed once all the nodes in the graph reach fixpoint. Since graph A does not contain any cycles(loops), post order algorithm traverses the graph in such a manner that each node will be visited only after their successors and the analysis will be completed in single traversal of the graph. Worklist approach too involves visiting the nodes only once but it also involves creation of worklist of size 100 which is an overhead. DFS and random traversals requires multiple traversal over the graph to complete the analysis. 

%Reverse post order algorithm performs better than other traversal strategies for \textit{dominator analysis} on graph A. This is because \textit{dominator analysis} is a forward data flow analysis and the output at each nodes in the graph are dependent on the output of their predecessor nodes. Since graph A does not contain any cycles(loops), reverse post order algorithm traverses the graph in such a manner that each node will be visited only after their predecessors and the analysis will be completed in single traversal of the graph.

%For \textit{used variable analysis}, random traversal works better than other traversal strategies for graph A. This is because \textit{used variable analysis} is a non data flow analysis and the output at each node is not dependent on output of other nodes and hence it is independent on the order of nodes visited. Therefore random traversal performs better than other traversal strategies.\newline

%For graph B, Figure \ref{fig:graphb} shows that worklist approach with worklist created by post ordering of nodes performs better for \textit{live variable analysis} and worklist approach with worklist created by reverse post ordering of nodes performs better for \textit{dominator analysis}. This is because graph B contains cycles(loops) and hence all traversal strategies except worklist requires multiple traversal over the whole graph B to reach fixpoint. This in-turn means visiting redundant nodes in each traversal iteration. Worklist visits only the nodes that have not reached fixpoint and does not visit redundant nodes and hence emerges as the better one among the traversal strategies. For \textit{used variable analysis}, random traversal performs better once again. This is because the output at each node is not dependent on output of other nodes and hence the cycles present in the graph does not affect this analysis.
%\newline
%From the above example, we can safely conclude that
%\begin{itemize}
%\item Given a graph,  no single traversal strategy is the best for all analysis.
%\end{itemize}
%Identifying best traversal strategy becomes really important when we analyze large scale software repositories which contains a variety of projects with methods with different characteristics, which warrants different traversal strategy for faster analysis. To illustrate, we ran 20 analysis on Dacapo dataset containing 280k methods using seven candidate traversal strategies. Figure (not yet provided) shows 20 stacked bar chart, one for each analysis. Each shaded area depicts the percentage of dataset on which that particular traversal strategy was the fastest to complete the analysis. One can see that no single traversal strategy is dominant across all analysis. The varying percentage of dominancy of each traversal strategies across the analysis indicates that
%\begin{itemize}
%\item Given a analysis,  no single traversal strategy is the best for all graphs.
%\end{itemize}

The analysis task that needs to be performed can have various characteristics(data flow analysis [5], data flow in-sensitive analysis, iterative analysis etc.) and the large scale data that the analysis has to be performed upon contains graphs of different characteristics and based on these analysis characteristics and graph characteristics, they may warrant a particular strategy.\newline
Our intuition is that the analysis code characteristics and the graph characteristics may lead us to the traversal strategy best suited for the analysis and the graph. Leveraging this information from analysis code statically and information from graph dynamically, we can apply the best traversal that needs fewer node visits and fewer operations per node to perform the analysis when compared to other traversal strategies.\newline

%\begin{figure}[t]
%  \centering
%  \includegraphics[width=4in]{tex-figures/motivation-bar.png}
%  \caption[Bar chart showing 20 stacked bars, one for each analysis. Each shaded area depicts the percentage of dataset on which that particular traversal strategy was the fastest to complete the analysis.]
%   {Bar chart showing 20 stacked bars, one for each analysis. Each shaded area depicts the percentage of dataset on which that particular traversal strategy was the fastest to complete the analysis.}
%\end{figure}

The next section describes the constructs that we are going to use describe our analysis. This construct will in-turn be used in our algorithms to analyze our analysis.


==> obey.tex <==
%{obey}

% \myobeycr is same as \obeycr, but doesn't do a \@gobblecr.
{\catcode`\^^M=13 \gdef\myobeycr{\catcode`\^^M=13 \def^^M{\\}}%
\gdef\restorecr{\catcode`\^^M=5 }}

% \obeytabs
{\catcode`\^^I=13 \gdef\obeytabs{\catcode`\^^I=13 \def^^I{\hbox{\hskip 4em}}}}

% \obeyspaces
{\obeyspaces\gdef {\hbox{\hskip0.5em}}}

% environment for displayed text, indented, obeys cr, tab, spaces
\newenvironment{obeyDisplay}{%
\samepage%
\begin{list}{}{}\item\obeyspaces\obeytabs\obeycr}{%
\end{list}}


==> overview-new.tex <==
\section{Approach Overview}
\label{sec:overview}
% 
% In this section we provide a brief overview of our hybrid technique for
% selecting optimal traversal strategy for analysis traversals.
% \fignref{fig:overview} provides an overview diagram of our approach.
\begin{figure*}[ht!]
  \centering \includegraphics[width=\linewidth]{figures/overview.pdf}
\caption{Overview of the hybrid approach for selecting and optimizing graph traversal strategy.}
  \label{fig:overview}
\end{figure*}

\fignref{fig:overview} provides an overview of our hybrid approach for selecting
and optimizing the traversal strategies for analysis traversals.
Inputs to our approach are analysis that contains one or more traversals, and a
graph. Output of our technique is an optimal traversal strategy for every
traversal in the analysis. For selecting an optimal traversal strategy for a
traversal, our technique computes a set of static properties of the traversal,
such as data flow sensitivity, loop sensitivity, and extracts a property about
the graph that defines the node connectivity in the graph
(sequential/branch/loop). Upon computing the static and dynamic properties, our
approach selects a traversal strategy from a set of candidate strategies for
each traversal in the analysis and optimizes it.

\subsection{Static Properties of Analysis Traversals}
\label{sec:static-properties}

\begin{definition}\label{def:dataflow}
\textbf{Data flow sensitivity} property $P_{DataFlow}$ is a property of a
traversal that indicates whether the traversal output of a node is dependent on
the traversal output of other nodes. The domain of values for $P_{DataFlow}$ are
\{\textit{true}, \textit{false}\}. If $O$ is a map that collects and maintains
the traversal output of nodes, $F$ is a function, and $O[n]$ = $F(O[n_p])$,
where $n_p \in n.preds$ or $n_p \in n.succs$, then $P_{DataFlow}$ =
\textit{true}.
\end{definition}

For instance, consider the lines 16 and 17 of the \lstinline|domT| traversal
shown in Listing \ref{lst:dominators}. Here, a variable \lstinline|dom| holds
the traversal output of a node $n$ and it is computed by applying an
\lstinline|intersection| operation on traversal outputs of predecessors of $n$.
Here, the function $F$ is \lstinline|intersection| over all predecessors of a
node.

To determine the data flow sensitivity property, the operations performed in the
traversal needs to be analyzed. An algorithm that analyzes the body of the
traversal to determine the data flow sensitivity property is provided in
\algoref{algo:flow-sensitive}.

\begin{definition}\label{def:loop-sensitivity}
\textbf{Loop sensitivity} property $P_{Loop}$ is a property of a data flow
sensitive traversal that indicates whether the data flow in the traversal
is affected by the loops (or cycles) present in the input graph. 
The domain of values for $P_{DataFlow}$ are \{\textit{true}, \textit{false}\}.
If a traversal is affected by the loops in the graph, the traversal requires
multiple iterations to compute output for nodes.
The traversal output either shrinks or expands before reaching a fix-point, if
it is affected by the loops. Hence, if the traversal output shrinks or expands
in the subsequent iterations, then the traversal is said to be loop sensitive.
If $O[n, i]$ represents the traversal output of a node $n$ in iteration $i$, and
if $O[n, i+1]$ $\lll$ $O[n, i]$ or $O[n, i+1]$ $\ggg$ $O[n, i]$, then $P_{Loop}$
= \textit{true}. The symbol $\lll$ represents \lstinline|shrink| and the symbol
$\ggg$ represents \lstinline|expand|. 
\end{definition}

Loop sensitivity is defined for only the data flow sensitive traversals (data
flow insensitive traversals do not have loop sensitivity property). When the
input graph contains loops, the traversal may or may not get affected by it. If
a traversal gets affected by the loops in the input graph, the traversal visits
nodes multiple times (requires multiple iterations) to stabilize the output and
reach a fix-point. To determine this statically, we assume that the traversal
takes multiple iterations (visits nodes multiple times), and we check if the
traversal output of nodes expands or shrinks in the subsequent iterations. If
the traversal output expands or shrinks in the subsequent iterations, we can
conclude that the traversal will get affected by the loops in the input graph.
The expand and shrink conditions are given by:  $O[n, i+1]$ $\lll$ $O[n, i]$ and
$O[n, i+1]$ $\ggg$ $O[n, i]$. For these conditions to hold, the conditions below
must also be true. \\
% 
% When the input graph contains loops, the traversal visits nodes multiple times
% to stabilize the output and reach a fix-point. A traversal is checked for loop
% sensitivity if the traversal is data flow sensitive, hence following conditions
% holds for a traversal to be loop sensitive: \\

$F(O[n_p]) \lll O[n_p]$ $\wedge$ $O[n_p, i+1] \lll O[n_p, i]$ $\Rightarrow$
$O[n, i+1] \lll O[n, i]$ \\
$F(O[n_p]) \ggg O[n_p]$ $\wedge$ $O[n_p, i+1] \ggg O[n_p, i]$ $\Rightarrow$
$O[n, i+1] \ggg O[n, i]$, where $n_p \in n.preds$ or $n_p \in n.succs$. \\

To give an example, consider the \lstinline|domT| traversal shown in Listing
\ref{lst:dominators}. For this traversal $P_{Loop}$ is \lstinline|false| and the
rationale is as follows. For this traversal, we want to check if the traversal
output shrinks or expands. The \lstinline|intersection| operation in line 17
always shrinks the output, hence the condition $F(O[n_p]) \lll O[n_p]$ is true,
where $F$ is \lstinline|intersection| operation. However, the second condition,
$O[n_p, i+1] \lll O[n_p, i]$ is \lstinline|false|, because in the body of the
traversal (lines 5-20), there exists no \lstinline|remove| operation, hence
between multiple iterations the output cannot shrink.

To determine if the traversal output expands or shrinks in the subsequent
iterations, the operations performed in the traversal needs to be analyzed.
A combination of operations like \lstinline|union| with \lstinline|add| suggests
that the traversal output expands, and a combination of operations like
\lstinline|intersection| with \lstinline|remove| suggests that the traversal
output shrinks. We provide an algorithm to determine this property by analyzing
the operations performed in the traversal body in \algoref{algo:loop-sensitive}.

% \subsection{Dynamic Properties of Graphs}
% \label{sec:dynamic-properties}
% Our approach requires classifying input graphs based on the connectivity of
% nodes.
% \begin{itemize}
%   \item {\em Sequential}: All nodes in the graph have single successor and
%   predecessor.
%   \item {\em Branch}: There exists nodes that have more than one successors or
%   predecessors.
%   \item {\em Loop}: There exists cycle(s) in the graph.
% \end{itemize}

% the nature of the control flow in it. Based on the nature of the control flow we
% classify graphs into:
% \begin{itemize}
%   \item {\em Sequential control flow}: CFG contains no branch instructions and
%   all nodes have single successor.
%   \item {\em Conditional branch control flow}: CFG contains branch instructions,
%   such as \lstinline|if-else|, \lstinline|switch-case|, etc, however no loop
%   instructions, such as \lstinline|for|, \lstinline|while|, etc, exists. 
%   \item {\em Loop based control flow}: CFG contains loop instructions.
%   \begin{itemize}
%     \item {\em With conditional branch}: CFG contains loop instructions and
%     branch instructions. 
%     \item {\em Without conditional branch}: CFG contains loop instructions, but
%     no branch instructions.
%   \end{itemize}
% \end{itemize}

\subsection{Selecting and Optimizing the Traversal Order}
\label{sec:select-optimize}

We model the selection of optimal traversal strategy using the decision tree
shown in \fignref{fig:decision-diagram}. Inputs to our decision tree are: a
traversal and a graph, and output is a traversal strategy selected from a list
of candidate traversal strategies shown in \tabref{tab:strategies}.
The decision tree checks both static properties about the traversal, and the
dynamic properties about the input graph~\footnote{Note that, when we say
dynamic properties about the input graph, we mean the connectivity of nodes in
the graph, which is available only at runtime}.
The static properties includes: data flow sensitivity, loop sensitivity, and
traversal direction. The dynamic property is the graph connectivity that
describes how nodes are connected to each others.
Based on connectivity, we classified graphs into: \{sequential, branch only,
loop w/o branch, loop w/ branch\}~\footnote{In case of sequential graphs, all
nodes in the graph have no more than one successor and predecessor. In case of graphs
with branches, nodes may have more than one successor or predecessor. In case of
graphs with loops, there exists cycles in the graph.}.

Here, we briefly describe the traversal strategy selection steps using the
\textit{Post-Dominator Analysis} given in Listing \ref{lst:dominators}, for
input graphs with different connectivity.
The \textit{Post-Dominator Analysis} contains two traversals:
\lstinline|initT| and \lstinline|domT|.
For \lstinline|initT| traversal, $P_{DataFlow}$ is \textit{false} and $P_{Loop}$
is \textit{false}, and for \lstinline|domT| traversal, $P_{DataFlow}$ is
\textit{true} and $P_{Loop}$ is \textit{false}. The traversal directions of
\lstinline|initT| and \lstinline|domT| traversals are \lstinline|ITERATIVE| and
\lstinline|BACKWARD| respectively.
The connectivity of input graphs can be anything in the set \{sequential, branch
only, loop w/o branch, loop w/ branch\}.
We now select an optimal traversal strategy for each of them.

The decision procedure begins by checking the data flow sensitivity property of
the traversal ($P_{DataFlow}$). For \lstinline|initT| traversal, $P_{DataFlow}$
is \textit{false}, hence \textit{SEQ} traversal strategy is picked as shown in
\fignref{fig:decision-diagram} and no further checking is required. The
traversal strategy \textit{SEQ} represents sequential order that visits nodes in
the order they appear in the nodes list.
For \lstinline|domT| traversal, $P_{DataFlow}$ is \textit{true}. The next static
propery to be checked is loop sensitivity property ($P_{Loop}$), however
$P_{Loop}$ is only applicable to graphs with loops, we check the connectivity
property of the input graph.
\begin{itemize}
  \item For graphs with sequential connectivity, we check the traversal
  direction and assign \textit{DEC} strategy (path $P_2$ in
  \fignref{fig:decision-diagram}). This is because, for sequential graphs, the
  traversal is expected to visit every node only once and visiting the nodes in
  the decreasing order of the node ids ensures that the graph is visited in
  the reverse order it was constructed. For instance, for visiting CFGs, the
  decreasing order of the node ids gives the reverse control flow order of
  nodes.
  The \textit{DEC} traversal strategy benefits traversals that have backward
  traversal direction. The \lstinline|domT| traversal is a backward traversal.
  \item For graphs with branch connectivity, \textit{PO} is
  picked for backward traversals (path $P_4$). This is because, in backward
  traversals, outputs of successors is required for computing the output at
  any node, and post order (\textit{PO}) visits all successors
  of a node before visiting that node, hence \textit{PO} is picked.
  \item For graphs with loop connectivity, loop sensitivity property
  ($P_{Loop}$) is checked. For \lstinline|domT| traversal, $P_{Loop}$ is
  \textit{false}. The next property to be checked is whether the graph also
  contains branches along with loop. This is because, for loop insensitive
  traversals, the loops in the input graph have no effect on the traversal order
  and the selection decision reduces to with or without branches. For graphs
  with branches, \textit{PO} is picked (path $P_6$), and for graphs without
  branches, \textit{DEC} is picked (path $P_8$). The reasoning is similar to the
  sequential and branch case described above.
\end{itemize}

To summarize, for \lstinline|initT| traversal, \textit{SEQ} traversal strategy
is picked (path $P_{11}$ in our decision tree shown in
\fignref{fig:decision-diagram}) and for \lstinline|domT| traversal, any of the
following strategies can be picked based on the graph connectivity:
\{\textit{DEC}, \textit{PO}\} (along paths $P_2$, $P_4$, $P_6$, $P_8$).
Further, our hybrid checking enables applying optimizations to the selected
traversal strategy. One such optimization is eliminating the fix point check for
graphs that are sequential. The fix point checking requires an additional
traversal of the graph, and for sequential graphs, the fix point check is not
needed, as the traversal only requires one iteration.


==> overview.tex <==
\section{Approach Overview}
\label{sec:approach-overview}

%\begin{figure*}[ht!]
 % \centering
  %\includegraphics[width=0.54\linewidth]{tex-figures/graph.png}
%\caption{Example graphs.}
 % \label{fig:example-graph}
%\end{figure*}

\begin{figure*}[ht!]
  \centering
  \includegraphics[width=\linewidth]{figures/overview.pdf}
\caption{Overview of the hybrid approach for selecting and optimizing graph traversal strategy.}
  \label{fig:overview}
\end{figure*}

Let us take the traverse operation in line 26 in the dominator analysis (Figure \ref{fig:dominator}) as our example traverse operation and a CFG with a loop and a branch \texttt{g} as our example CFG. The traverse operation applies the \texttt{dom\_T traversal} on \texttt{g} and is called with a fix-point \texttt{fp} with \texttt{FORWARD} traversal direction. We need to come up with the best traversal strategy to traverse \texttt{g} that completes the traverse operation faster than the other candidate traversal strategies. The overview of the hybrid approach for selecting and optimizing the graph traversal strategy is shown in Figure \ref{fig:overview}.

\subsection{Step 1 : Extract static properties from the traversal}
The first step is to analyze the traversal that is given as input in the traverse operation and extract the required static properties that we need, in-order to make the best traversal strategy decision. The required static properties are \textit{data flow sensitivity} of the traversal,% \textit{traversal sensitivity} of the traversal,% 
\textit{loop sensitivity} of the traversal and the \textit{traversal direction}.

%\begin{definition}
%\textbf{Traversal sensitivity} property is a property of the traversal that indicates whether the traversal is sensitive to the traversal strategy used to traverse the CFG and the result generated by the traversal at each node differs from one traversal strategy to another. If the traversal contains non commutative operations involving global variable, then such traversals are \textbf{traversal sensitive}.
%\end{definition} 
%\texttt{dom\_T} traversal in \textit{dominator analysis} does not contain any non commutative property involving global variable and hence it is determined as \textit{traversal in-sensitive}.
\begin{definition}
\textbf{Data flow sensitivity} property is a property of the traversal that indicates whether the traversal output of a node is dependent on the traversal output of other nodes. In line 13-14 of the dominator traversal, the \texttt{dom}
variable of current node n is dependent on the traversal output
of its predecessors. Hence \texttt{dom\_T} traversal in \textit{dominator analysis}
is data flow sensitive. Data flow sensitive traversal usually requires multiple traversal over the CFG untill all nodes reach fix-point ie the output of the nodes stabilizes.
\end{definition} 

\begin{definition}
\textbf{Loop sensitivity} property is a property of the data flow sensitive traversal that indicates whether the data flow in the traversal is affected by the loops present in the CFG. In data flow sensitive traversals, a node's output is dependent
on its neighbor's(successor/predecessor) output. If a back edge is present in the graph, then the back edge's destination
node will be visited before back edge's source node. Since the source node's output will not be available, the destination
node's output cannot be computed in the current traversal of the CFG
and hence another traversal is needed. Now we have to determine whether the traversal really needs the source node's
output to compute the destination node's output. From line 14 in \texttt{dom\_T} traversal, we can see that
\texttt{intersection} is used to merge the current node's traversal output with
its neighbor's traversal output. \texttt{Intersection} only shrinks a node's traversal output from one iteration to another. In this case, a back edge's
source node's traversal output can affect the back edge's destination
node's traversal output only if some element has been removed from the traversal output of
the source node, because only when an element is removed,
the set can further shrink in intersection and newly added elements does not affect in intersection operation. In \texttt{dom\_T} traversal of \textit{dominator analysis}, we can see that no element is removed from
the traversal output during the traversal and hence we can conclude that \texttt{dom\_T} traversal is \textit{loop insensitive}.
\end{definition}
Analysis direction is extracted from the traverse operation argument. In line 26 of the \texttt{dom\_T} traversal in \textit{dominator analysis}, we see that the analysis direction is \texttt{FORWARD}.
Hence we conclude that \texttt{dom\_T traversal} in \textit{dominator analysis} is \textit{%traversal in-sensitive,
	forward data flow sensitive and loop in-sensitive traversal}.

\subsection{Step 2 : Extract dynamic properties from the CFG}
The next step is to extract the required dynamic properties from the CFG \texttt{g}. The only property that is of interest to us is the type of control flow present in the CFG.
We classify CFGs into three types(\textit{Sequential CFG, CFG with branches and no loops, CFG with loops}) based on their control flow.
\begin{definition}
\textbf{Sequential CFG} are CFGs that does not have any branches or loops.
\end{definition}
\begin{definition}
\textbf{CFG with branches and no loops} are CFGs which have branches but no loops.
\end{definition}
\begin{definition}
\textbf{CFG with loops and no branches} are CFGs that has loops and do not contain any other branches.
\end{definition}
\begin{definition}
	\textbf{CFG with loops and branches} are CFGs that has loops and contains branches apart from the loops.
\end{definition}
Our input CFG \texttt{g} is a \textit{CFG with loops and branches}.

\subsection{Step 3 : Traversal strategy decision}
\begin{itemize}
%\item We first check whether our traversal is \textit{traversal sensitive} or not. If the traversal is sensitive to the traversal strategy used, the result of the traversals differs based on the used traversal strategy and hybrid approach cannot make decision for such traversals. Our example traversal, which is \texttt{dom\_T} traversal in \textit{dominator analysis} is \textit{traversal in-sensitive} and hence hybrid approach is applicable and we will choose the best traversal strategy that will finish the analysis faster.
\item The first step is to check whether our traversal is \textit{data flow sensitive} or not. We check this property because \textit{data flow sensitive} traversal requires multiple traversals over the CFG and hence we will try to choose the traversal strategy that visits lesser number of nodes and also does lesser number of operations per node. 
%\textit{Data flow in-sensitive} analysis requires single traversal of the CFG and hence we will choose the traversal strategy that does lesser number of operations per node. 
We have determined that \texttt{dom\_T} traversal is \textit{data flow sensitive}. In these kind of traversal, where traversal output at one node is dependent on traversal output of other nodes, a simple way to perform these traversal is to set up flow equations for each node of the CFG and solve them by repeatedly calculating the output from the input at each node until all the nodes reaches a fix-point. In order for all the nodes to reach fix-point, it may require multiple traversals over the CFG which is determined by the CFG structure.
\item We have determined that our CFG \texttt{g} contains loops. For CFGs containing loops, no traversal strategy can give a ordering of nodes that could solve the data flow sensitive traversal in a single traversal of the CFG. We now have to investigate whether the loop present in \texttt{g} affects the number of traversals in our data flow sensitive traversal.
\item We have determined that \texttt{dom\_T} traversal is \textit{loop in-sensitive} and therefore the loops present in \texttt{g} is not going to affect the data flow. We now investigate whether \texttt{g} contains any branches apart from the loops present. Our CFG does contain a branch. 
\item We then look at the \textit{traversal direction} and we have determined it to be \texttt{FORWARD}. For \textit{forward data flow sensitive} traversal, a traversal strategy can complete it in one traversal of the CFG only if the nodes are visited in such a way that each node is visited only after the node's predecessors. \textit{Reverse post-order} traversal guarantees such ordering of  nodes when CFG contains only branches. Though our CFG contains loop, we can ignore the loop present in our CFG as it does not affect the data flow. Without the loop, our CFG contains only branches and hence \textit{Reverse post-order} traversal will be chosen as the traversal strategy as it provides us with an ordering of nodes such that the analysis will reach fix-point in single traversal of the CFG.
%\item So for this CFG \texttt{g} and traversal \texttt{dom\_T}, the best traversal strategy is to visit the nodes in the increasing order of node ids since the node ids are assigned in a topological order. Traversing a sequential CFG in increasing topological order makes sure that a node is visited after its predecessors and hence we will complete the \texttt{dom\_T} traversal in a single traversal of the CFG. 
\item The next step is to optimize the chosen traversal strategy. We do not need fix-point checking operation to be done, as we knew from the static and dynamic properties that the traversal will be completed in single traversal and we do not need to check fix-point for each node to confirm. Hence we optimize the chosen traversal strategy to remove fix-point checking operation. Hence we visited the minimum number of nodes and also reduced the number of operations per node.
\end{itemize}
This is only one path to the traversal strategy decision in the decision tree and there exists many other paths which is shown in Figure \ref{fig:decision-tree}. The next section lists the candidate traversal strategies and explains our approach and the decision tree.

==> overview_decision.tex <==
\begin{figure*}[ht!]
\centering
\begin{minipage}{\linewidth}
\centering
  \includegraphics[width=0.48\textwidth]{tex-figures/overview_picture.png}
  \caption[Hybrid approach overview picture]
   {Hybrid approach overview picture}
\label{fig:overview}
\end{minipage}
\begin{minipage}{\linewidth}
\centering
  \includegraphics[width=\textwidth]{tex-figures/decision_tree.png}
  \caption[Decision tree - the path to picking best traversal]
   {Decision tree - the path to picking best traversal}
  \label{fig:decision}
\label{fig:cluster_df}
\end{minipage}
\end{figure*}


==> paper.tex <==
% PaperOnly are included in this paper
\newcommand{\PaperOnly}[1]{#1}
%
% TROnly are ignored in this paper
\newcommand{\TROnly}[1]{\relax}

\input{main-icse.tex} 


==> related.tex <==
\section{Related Work}
\label{sec:related}

To the best of our knowledge, our proposal to leverage information about the
program analysis code, and the nature of the data on which analysis is applied
to select appropriate traversal strategies has not been explored previously.
Below we discuss works that are related to various aspects of our proposal. 

\emph{Mixing static and dynamic information.} %
The general philosophy of mixing static and dynamic information has a long 
history~\cite{Ernst2003} in both the software engineering and the programming 
languages communities, with examples such as DSD-Crasher~\cite{DSD-Crasher}, 
Palus~\cite{Palus}, segmented symbolic execution~\cite{Le2013}, guided 
dynamic symbolic execution~\cite{Christakis2016}, gradual typing~\cite{Siek07}
, hybrid type checking \cite{Flanagan06}, intensional polymorphism~\cite{Harper95, 
Crary98}, etc. While our proposal also mixes static information 
about program analysis with dynamic information about the data, none of the 
previous works have proposed utilizing this information for selecting 
appropriate traversal strategies for realizing the program analysis.

\emph{Optimizing program analysis.}%
Atkinson ~\cite{atkinson2001implementation} presented techniques that reduce 
the time and space required to perform data-flow analysis of large programs. 
While their techniques proposed modifications to the underlying data-flow 
analyses that yield improvement in performance and also proposed reclamation 
of the data-flow sets during data-flow analysis that result in saving space, 
hybrid approach gives performance gain by analyzing the user written 
algorithm and the input graph received.\newline Kildall ~\cite{kildall1973unified} 
presented an algorithm which, in conjunction with various optimizing 
functions, provides global program optimization, Optimizing functions have 
been described which provide constant propagation, common sub-expression 
elimination, and a degree of register optimization. While their approach 
provides unified approach to global program optimization, we concentrate on 
optimizing the process that does program optimization using the program's 
structure and the algorithms characteristics.

\emph{Ultra-large-scale source code mining.}%
In terms of ultra large scale processing, Boa~\cite{dyer2013boa} is a 
language and infrastructure for analyzing ultra-large-scale software 
repositories. Boa provides a different kind of performance gain through its 
infrastructure and eases testing MSR-related hypotheses, it is not suitable 
for graph processing algorithms and does not leverage information from 
algorithms written in Boa.

\emph{Graph traversal optimization.}%
There have been many works that targeted graph traversal optimization through 
various ways. Green-Marl~\cite{hong2012green} provides performance benefits 
by using domain specific knowledge in applying optimizations. It uses high-level 
algorithmic description written in Green-Marl to exploiting the exposed 
data level parallelism. While green marl provides performance benefits by 
taking algorithm written into consideration, hybrid approach takes both 
algorithm and graph structure into account. And in ultra large scale dataset, 
containing millions of graphs with different structures, the gain that we can 
incur by taking graph structure into account is significant.

Pregel~\cite{malewicz2010pregel} is a MapReduce like framework that aims to 
bring distributed processing to graph algorithms. While Pregel's performance 
gain is through parallelism and handles large graphs processing through 
vertex centric approach, our approach achieves performance gain by traversing 
the graph efficient suitable to the algorithm.

There have also been few libraries that support parallel or distributed graph 
analysis: Parallel BGL~\cite{gregor2005parallel}  is a distributed version of 
BGL while SNAP~\cite{bader2008snap}  is a stand-alone parallel graph analysis 
package.
% TODO - text below requires huge amount of editing.
% Organize under the categories given above.


==> static-prop.tex <==
\subsection{Computation of static properties}
\label{sec:static}
\input{tex-figures/algorithms/flow_sensitivity.tex}
\input{tex-figures/algorithms/loop_sensitivity.tex}
%\input{tex-figures/algorithms/traversal_sensitivity.tex}
Properties of the traversal are computed by performing analysis over the control-flow graph representation of the traversal. The required static properties are data flow sensitivity, loop sensitivity and traversal direction.
%\begin{definition}
%A \textbf{Control Flow Graph (CFG)} of a program is defined as $G$ = $(N, E,
%\top, \bot)$, where G is a directed graph with a set of nodes N representing
%program statements and a set of edges E representing the control flow between
%statements. $\top$ and $\bot$ denote the start and end nodes of the graph.
%\end{definition}

%\subsubsection{Property 1 :  Data flow sensitivity}
%\label{sec:dataflow}
%\begin{definition}
%If an analysis at a node in a graph is dependent on the analysis output of other %nodes, then
%such analysis are said to be \textbf{Data flow sensitive}. Analysis that are
%sensitive to the informations flowing through the graph are
%said to be data flow sensitive analysis. Consider \textit{live\_analysis} traversal
%in live variable analysis in Figure \ref{fig:live-variable}. In line 17 and 18, the $live$
%variable of current node n is dependent on the $live$ variable
%of its successors. Hence \textit{live\_analysis traversal} in live variable analysis
%is data flow sensitive.
%\end{definition}

\subsubsection{Determining data flow sensitivity}
\label{sec:determine-dataflow}
Given a traversal \texttt{t := traversal(n : Node) : OType \{ tbody \}} where $t$ is the traversal identifier, $n$ is the input node, $OType$ is the output type and $tbody$ is the traversal body, Algorithm \ref{algo:flow-sensitive} returns a boolean variable indicating data flow sensitivity of the traversal. $True$ indicates \textit{data flow sensitive}. The algorithm initially gets the control flow graph of the $tbdoy$ using the \textit{getcfg} function in line 1. Line 2 computes all the aliases of $n$ using the \textit{getAliases} function. \textit{getAliases} performs local may alias on CFG $G$ and returns the aliases of $n$. We then traverse the CFG $G$ node by node. Line 4 checks if any node contains a \textit{METHODCALL} statement and if it is, we get the method name of the method call using auxiliary function \textit{getMethod} in Line 5. If the method call is output($n'$, $t'$), then we determine that the traversal is trying to get the traversal output of node $n'$ of traversal $t'$. Line 6 then determines whether $t'$ is equal to $t$, which then indicates that the traversal is accessing the traversal output of node $n'$ of the current traversal $t$. Line 7 checks if $n'$ does not belong to the alias of the current node $n$. If true, then we determine that the traversal needs the traversal output of nodes other than the current node $n$ of the current traversal $t$. Hence we conclude that the traversal is \textit{data flow sensitive}.

%\subsubsection{Property 2 :  Loop sensitivity}
%\label{sec:loop}
%\begin{definition}
%Loops in data flow analysis affect the number of traversals needed over the graph. But some data flow analysis are
%not affected by the loops present and we term these analysis as \textbf{loop in-sensitive} data flow analysis. If loops dictates the number of traversal needed over the graph, then such analysis are termed as \textbf{loop sensitive} data flow analysis. In data flow analysis, a node's output is dependent
%on its neighbour's(successor/predecessor) output. If a back edge is present in the graph, then the back edge's destination
%node will be visted before back edge's source node. Since the source node's output will not be available, the destination
%node's output cannot be computed in the current traversal
%and hence another traversal is needed. Now we have to determine whether the %analysis really needs the source node's
%output to compute the destination node's output. Look at the
%\textit{dominator} traversal in dominator analysis in Figure \ref{fig:dominator}. From line 10, we can see that
%\textit{intersection} is used to merge the current node's output with
%its neighbors output. \textit{Intersection} only shrinks a node's output from one iteration to another. In this case, a back edge's
%source node's output can affect the back edge's destination
%node's output only if some element has been removed from
%the source node, because only when an element is removed,
%the set can further shrink in intersection and newly added elements does not affect in intersection. In \textit{dominator} traversal of dominator analysis, we can see that no element is removed from
%the output during the analysis and hence we can conclude that \textit{dominator} traversal block is \textit{loop insensitive}. In \textit{live\_analysis} traversal block of live variable analysis(Figure \ref{fig:live-variable}), we can see that \textit{union} is used for merging(line 18)
%and for union merge type, only the new elements added to the neighbors can affect the current node's output. From line 22,
%we see that new elements are added to node's output during the analysis and hence \textit{live\_analysis} traversal block in live variable analysis is
%\textit{loop sensitive}.
%\end{definition}
\subsubsection{Determining loop sensitivity}
\label{sec:determine-loop}
Given a traversal \texttt{t := traversal(n : Node) : OType \{ tbody \}} where $t$ is the traversal identifier, $n$ is the input node, $OType$ is the output type and $tbody$ is the traversal body, Algorithm \ref{algo:loop-sensitive} returns a boolean variable indicating loop sensitivity of the traversal. $True$ indicates \textit{loop sensitive}. The algorithm initially gets the control flow graph of $tbody$ using the \textit{getcfg} function. Line 2 computes all the aliases of $n$ using the \textit{getAliases} function. We then traverse the CFG $G$ node by node. Line 9-17 collects $lhs$ of expressions whose $rhs$ is \textit{output($n'$, $t'$)} and $t'$ is equal to $t$. This collection is partioned into $V$ and $V'$. $V$ contains all $lhs$ when $n'$ is an alias of node $n$ and $V'$ contains all lhs when $n'$ is not an alias of node $n$. Basically $V$ contains all variables whose value is the traversal output of the current traversal $t$ on current node $n$. $V'$ contains all variables whose value is the traversal output of the current traversal $t$ on other nodes. Once we have $V$ and $V'$, we traverse all the nodes once more. Line 21-24 checks whether the node contains \textit{union($C1$, $C2$)} method call. If true, we try to determine if one of the collections belong to $V$  and the other collection belongs to $V'$. This basically tells that union has been performed as merging of the current node's traversal output and some other node's traversal output. Hence we add \textit{union} as a merge operation. Here $M$ collects all the merge operation. \textit{Intersection} is also checked in the same way (Line 26-30).\par 
In line 31-35, we check if node contains either \textit{add($C1$, $e$)} or \textit{addAll($C1$, $C2$)} method call. If true, we check whether $C1$ is a part of $V$, ie whether $C1$ is a collection that contains traversal output of the current node $n$. If true, it indicates that some information is being added to the traversal output of the current node $n$ and we mark that using $genFlag$ in line 33. Similary in line 36-40, we check if node contains either \textit{remove($C1$, $e$)} or \textit{removeAll($C1$, $C2$)} method call. If true, we check whether $C1$ is a part of $V$, ie whether $C1$ is a collection that contains traversal output of the current node $n$. If true, it indicates that some information is being removed from the traversal output of the current node $n$ and we mark that using $killFlag$ in line 38. 
Line 43-48 concludes that the traversal is \textit{loop sensitive} if either the traversal has union merge operation and the $genFlag$ set or it has intersection merge operation and $killFlag$ set. In all other cases, it is \textit{loop insensitive}.

%\subsubsection{Property 3 :  Traversal sensitivity}
%\label{sec:traversal}
%\begin{definition}
%\textbf{Traversal sensitive} analysis are analysis that are sensitive to the traversal strategy used and the results of the analysis differ from one traversal strategy to another. If the traversal block contains non commutative operations involving global variable, then such traversal blocks are \textbf{traversal sensitive}.
%\end{definition}

%\paragraph{Determining traversal sensitivity}
%Given a traversal block with its identifier $t$ and input node $n$ and Global variables $GV$ of the program, Algorithm \ref{algo:traversal-sensitive} returns a boolean variable indicating the traversal sensitivity of the traversal block. $True$ indicates \textit{traversal sensitive}. The algorithm initially gets the control flow graph of the traversal block's body using the \textit{getcfg} function in line 1. We then traverse the CFG $G$ node by node. Line 4 checks if the node contains either \textit{add($C1$, $e$)} or \textit{addAll($C1$, $C2$)} method call. If it does, Line 5 checks if $C1$ is a global variable of type sequence, then we conclude it as \textit{traversal sensitive}. This is because \textit{Sequence} is order dependent data type and adding elements in different order will provide different ordering of elements in \textit{Sequence} data type, while this is not the case in \textit{Set} data type as any order of adding elements will produce the same state. Line 9 checks whether the method call is \textit{hasElement($C1$, $e$)} or \textit{equals($C1$, $C2$)}. If so, we check if $C1$ is a global variable. If true, then we conclude the traversal block is \textit{traversal sensitive}. This is because operations like \textit{hasElement} and \textit{equals} produce non-commutative results and hence the presence of these operations on global variable makes the traversal sensitive to the traversal strategy used. Line 15-23 checks if the node is an $lhs$ = $rhs$ statement and if $lhs$ is an global variable and $rhs$ contains a non global varaiable, then the traversal block is \textit{traversal sensitive}. This is because if global variable is assigned using a local variable, then the last traversed node will affect the value of $lhs$ and hence it is \textit{traversal sensitive}.

\subsection{Computation of dynamic properties}
\label{sec:dynamic}
The only dynamic property that we need from the input CFG is whether it contains
branches and loops. Since CFG is the representation of a program, these
properties could be determined while creation of the CFG. Since CFGs are
constructed by parsing the expressions and the statements in the program, we can
see that for a given language, only certain constructs, for example - “While”,
“For” in Java create loops. For a given language, it is easy to enumerate the
constructs in the language that generate loops and branches. And while creating
the CFG, when the construct that generates loop is encountered, then the CFG is
marked as containing loops. Similarly when the construct that generates branch
is encountered, then the cfg is marked as containing branches.
Hence the dynamic properties are affixed to the CFG during its creation.

==> tex-figures/accuracy_table.tex <==

\begin{figure}[t]
\begin{footnotesize}
\begin{tabular}{ | c | c |}
\hline
\textbf{Analysis} & \textbf{Accuracy of results} \\ \hline
AE	& 100\% \\ \hline
CSE	& 100\% \\ \hline
CP	& 100\% \\ \hline
DC	& 99.999\% \\ \hline
DOM	& 99.999\% \\ \hline
LV	& 99.999\% \\ \hline
LMA	& 99.991\% \\ \hline
LMNA	& 100\% \\ \hline
LIC	& 100\% \\ \hline
NA	& 100\% \\ \hline
PDOM	& 99.999\% \\ \hline
RD	& 100\% \\ \hline
USA	& 100\% \\ \hline
VBE	& 100\% \\ \hline
RS	& 99.994\% \\ \hline
IL	& 100\% \\ \hline
UIR	& 100\% \\ \hline
UDV	& 100\% \\ \hline
WNIL	& 100\% \\ \hline
DSWI	& 100\% \\ \hline
\end{tabular}
\end{footnotesize}
\caption{Table showing accuracy of our result while adopting hybrid approach.}
\end{figure}


==> tex-figures/algorithms/dominator.tex <==
\begin{figure}[ht!]
% \centering
\begin{lstlisting}[numbers=left, tabsize=4, escapechar=@, caption={Dominator analysis: an example program analysis expressed using our
system.},label={lst:dominators}] 
allNodes : Set<int>;

initT := traversal (n : Node) { 
	add(allNodes, n.id);
}

domT := traversal (n : Node) : Set<int> { 
	Set<int> dom;
	if(output(n, domT) == null)
		dom = allNodes;
	else
		dom = output(n, domT);
	foreach(p : n.preds) 
		dom = intersection(dom, output(p, domT)) 
	add(dom, n.id); 
	return dom; 
} 

fp := fixp(Set<int> curr, Set<int> prev) : bool {
	if(equals(curr, prev))
		return true;
	return false;
}

traverse(g, initT, ITERATIVE); @\label{line:traverse}@
traverse(g, domT, FORWARD, fp); 				
\end{lstlisting}
% \caption{}
% % 
% % 
% % Dominator analysis performs traversal over the graph to determine the
% % dominators of each node. It has two traversals. \textit{init} traversal collects
% % all node ids. \textit{dom\_T} is called with a fixpoint and it runs till all the
% % nodes reach the fixpoint condition.}
% \label{fig:dominator}
\end{figure}




==> tex-figures/algorithms/live-variable.tex <==
\begin{figure}[ht!]
\centering
\begin{lstlisting}
2  killT := traversal (n : Node) : string { 
3  	if(n.stmt.kind == VARDECL || n.statement.kind == ASSIGNMENT) { 
4		return n.stmt.lhs; 
5	} 
6	return null; 
7  } 

8  genT := traversal (n : Node<P>) : Set<String> { 
9	return n.stmt.rhs.variables; 
10 } 


11 liveT := traversal (n : Node) : Set { 
12	live := output(n, liveT); 
13	kill := output(n, killT); 
14	gen := output(node, genT);  
15	foreach(s : node.succs) {
16		s_live := output(s, liveT);
17		live.out = union(live.out, s_live.in); 
18	}
19	live.in = live.out; 
20	remove(live.in, kill); 
21	addAll(live.in, gen); 
22	return live; 
23 }

24 fp := fixp(Set<string> out, Set<string> prev_out) : bool {
25	if(equals(out, prev_out))
26		return true;
27	return false;
28 }

29 traverse(g, killT, FORWARD, null);
30 traverse(g, genT, FORWARD, null); 
31 traverse(g, liveT, BACKWARD, fp); 				
\end{lstlisting}
\caption{Live variable analysis performs traversal over the graph to determine the live variables at each node. In \textit{kill\_traversal}, output of each node is the variable defined in it. In \textit{gen\_traversal}, output of each node is the variable used in it. The \textit{live\_analysis} traversal is the traversal which performs the live variable analysis. This traversal is called with fixpoint function as it is a data flow analysis and runs till the fixpoint is reached.}
\label{fig:live-variable}
\end{figure}


==> tex-figures/algorithms/traversal_sensitivity.tex <==
\begin{algorithm}
\KwIn{t := traversal(n : Node) : OType \{ tbody \}, GlobalVariables $GV$}
\KwOut{\textit{true/false}}
$G$ $\leftarrow$ \textit{getcfg($tbody$)}\;
\ForEach{ $node \in G.nodes$ }{
	\If{$node.stmt$ is of kind $METHODCALL$}{
		\If{\textit{getMethod($node.stmt$)} $\in$ \{\textit{add($C1$, $e$), addAll($C1$, $C2$)}\}}{
			\If{$C1$ $\in$ $GV$ and $C1$ is of type $Sequence$}{ 
				\textit{return true}\;
			}
		}\If{\textit{getMethod($node.stmt$)} $\in$ \{\textit{has($C1$, $e$), equals($C1$, $C2$)}\}}{
			\If{$C1$ $\in$ $GV$ || $C2$ $\in$ $GV$}{ 
				\textit{return true}\;
			}
		}
	}
	\If{$node.stmt$ is of kind $lhs = rhs$}{
		\If{$node.stmt.lhs \in GV$}{
			\ForEach{$v \in node.stmt.rhs$}{
				\If{$v$ $\notin$ $GV$}{ 
					\textit{return true}\;
				}
			}
		}
	}
}
\textit{return false}\;
\caption{Algorithm to detect traversal sensitivity}
\label{algo:traversal-sensitive}
\end{algorithm}


==> tex-figures/analysis_table-V1.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
	\footnotesize
  \centering
  \caption{List of program analyses and the properties of their involved traversals.}
    \resizebox{\textwidth}{!}{\begin{tabular}{|l|c|c|c|c|c|}
    \hline
    \multirow{3}[6]{*}{\textit{\textbf{Analysis}}} & \multirow{2}[4]{*}{\textit{\textbf{No of traversals}}} & \multicolumn{3}{c|}{\textit{\textbf{Type of traversal Involved}}} & \multirow{2}[4]{*}{\textit{\textbf{Traversal}}} \\
\cline{3-5}          &       & \multicolumn{2}{c|}{\textit{\textbf{Data flow sensitive}}} & \textit{\textbf{Data flow}} &  \\
\cline{3-4}          & \textit{\textbf{involved}} & \textit{\textbf{Loop sensitive}} & \textit{\textbf{Loop insensitive}} & \textit{\textbf{insensitive}} & \textit{\textbf{direction}} \\
    \hline
    Available expression (AE) & 1     & 1     & 0     & 0     & FORWARD \\
    \hline
    Copy propagation (CP) & 2     & 1     & 0     & 1     & FORWARD \\
    \hline
    Common sub-expression detection (CSD) & 2     & 1     & 0     & 1     & FORWARD \\
    \hline
    Dead code (DC) & 2     & 1     & 0     & 1     & BACKWARD \\
    \hline
    Dominator (DOM) & 1     & 0     & 1     & 0     & FORWARD \\
    \hline
    Loop invariant code (LIC) & 3     & 1     & 0     & 2     & FORWARD \\
    \hline
    Local may alias (LMA) & 1     & 1     & 0     & 0     & FORWARD \\
    \hline
    Local must not alias (LMNA) & 1     & 1     & 0     & 0     & FORWARD \\
    \hline
    Live variable (LV) & 1     & 1     & 0     & 0     & BACKWARD \\
    \hline
    Nullness analysis (NA) & 1     & 1     & 0     & 0     & FORWARD \\
    \hline
    Post-dominator (PDOM) & 1     & 1     & 1     & 0     & BACKWARD \\
    \hline
    Reaching definition (RD) & 1     & 1     & 0     & 0     & FORWARD \\
    \hline
    Resource status (RS) & 1     & 1     & 0     & 0     & FORWARD \\
    \hline
    Used and defined variable (UDV) & 1     & 0     & 0     & 1     & NO DIRECTION \\
    \hline
    Useless increment in return (UIR) & 1     & 0     & 0     & 1     & NO DIRECTION \\
    \hline
    Upsafety analysis (USA) & 3     & 1     & 0     & 2     & FORWARD \\
    \hline
    Very busy expression(VBE) & 1     & 1     & 0     & 0     & BACKWARD \\
    \hline
    Wait not in loop (WNIL) & 1     & 0     & 0     & 1     & NO DIRECTION \\
    \hline
    \end{tabular}}
  \label{tab:analysis-table}%
\end{table}%


==> tex-figures/analysis_table-V2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{table}[htbp]
	\footnotesize
  \centering
  \caption{List of program analyses and the properties of their involved traversals.}
    \begin{tabular}{|c|l|c|c|c|c|c|}
    \hline
    \textit{\textbf{$\#$}} & \textit{\textbf{$Analysis$}} & \textit{\textbf{\#$\tau$}} & \textit{\textbf{$\tau$}} & \textit{\textbf{$P_{DataFlow}$}} & \textit{\textbf{$P_{Loop}$}} & \textit{\textbf{$\DH$}} \\
    \hline
    1     & Available expression (AE) & 1    & $t_{0}$    & \checkmark    & \checkmark    & $\uparrow$ \\
    \hline
    \multirow{2}[4]{*}{2} & \multirow{2}[4]{*}{Copy propagation (CP)} & \multirow{2}[4]{*}{2} & $t_{0}$    & \checkmark    & \checkmark    & $\uparrow$ \\
\cline{4-7}          &       &       & $t_{1}$    & 0     & 0     & | \\
    \hline
    \multirow{2}[4]{*}{3} & \multirow{2}[4]{*}{Common sub-expression detection (CSD)} & \multirow{2}[4]{*}{2} & $t_{0}$    & \checkmark    & \checkmark    & $\uparrow$ \\
\cline{4-7}          &       &       & $t_{1}$    & 0     & 0     & | \\
    \hline
    \multirow{2}[4]{*}{4} & \multirow{2}[4]{*}{Dead code (DC)} & \multirow{2}[4]{*}{2} & $t_{0}$    & \checkmark    & \checkmark    & $\downarrow$ \\
\cline{4-7}          &       &       & $t_{1}$    & 0     & 0     & | \\
    \hline
    5     & Dominator (DOM) & 1    & $t_{0}$    & \checkmark    & 0     & $\uparrow$ \\
    \hline
    \multirow{3}[6]{*}{6} & \multirow{3}[6]{*}{Loop invariant code (LIC)} & \multirow{3}[6]{*}{3} & $t_{0}$    & 0     & 0     & | \\
\cline{4-7}          &       &       & $t_{1}$    & \checkmark    & \checkmark    & $\uparrow$ \\
\cline{4-7}          &       &       & $t_{2}$    & 0     & 0     & | \\
    \hline
    7     & Local may alias (LMA) & 1    & $t_{0}$    & \checkmark    & \checkmark    & $\uparrow$ \\
    \hline
    8     & Local must not alias (LMNA) & 1    & $t_{0}$    & \checkmark    & \checkmark    & $\uparrow$ \\
    \hline
    9     & Live variable (LV) & 1    & $t_{0}$    & \checkmark    & \checkmark    & $\downarrow$ \\
    \hline
    10    & Nullness analysis (NA) & 1    & $t_{0}$    & \checkmark    & \checkmark    & $\uparrow$ \\
    \hline
    11    & Post-dominator (PDOM) & 1    & $t_{0}$    & \checkmark    & 0     & $\downarrow$ \\
    \hline
    12    & Reaching definition (RD) & 1    & $t_{0}$    & \checkmark    & \checkmark    & $\uparrow$ \\
    \hline
    13    & Resource status (RS) & 1    & $t_{0}$    & \checkmark    & \checkmark    & $\uparrow$ \\
    \hline
    14    & Used and defined variable (UDV) & 1    & $t_{0}$    & 0     & 0     & | \\
    \hline
    15    & Useless increment in return (UIR) & 1    & $t_{0}$    & 0     & 0     & | \\
    \hline
    \multirow{3}[6]{*}{16} & \multirow{3}[6]{*}{Upsafety analysis (USA)} & \multirow{3}[6]{*}{3} & $t_{0}$    & 0     & 0     & | \\
\cline{4-7}          &       &       & $t_{1}$    & \checkmark    & \checkmark    & $\uparrow$ \\
\cline{4-7}          &       &       & $t_{2}$    & 0     & 0     & | \\
    \hline
    17    & Very busy expression(VBE) & 1    & $t_{0}$    & \checkmark    & \checkmark    & $\downarrow$ \\
    \hline
    18    & Wait not in loop (WNIL) & 1    & $t_{0}$    & 0     & 0     & | \\
    \hline
    \end{tabular}%
  \label{tab:analysis-table}%
\end{table}%


==> tex-figures/error_table.tex <==

\begin{figure}[t]
\begin{footnotesize}
\begin{tabular}{ | c | c | c |}
\hline
\textbf{Analysis} & \textbf{Error Rate} & \textbf{Impact(ms)} \\ \hline
AE	& 0.06\%	& 198 \\ \hline
CSE	& 0.10\%	& 252 \\ \hline
CP	& 0.14\%	& 7316 \\ \hline
DC	& 0.07\%	& 371 \\ \hline
DOM	& 0.03\%	& 108 \\ \hline
LV	& 0.09\%	& 803 \\ \hline
LMA	& 0.27\%	& 203 \\ \hline
LMNA	& 0.27\%	& 4547 \\ \hline
LIC	& 0.16\%	& 1718 \\ \hline
NA	& 0.11\%	& 203 \\ \hline
PDOM	& 0.02\%	& 225 \\ \hline
RD	& 0.27\%	& 7169 \\ \hline
USA	& 0.05\%	& 195 \\ \hline
VBE	& 0.03\%	& 454 \\ \hline
RS	& 0.17\%	& 396 \\ \hline
IL	& ~0\%	& 0.087 \\ \hline
UIR	& ~0\%	& 0.02 \\ \hline
UDV	& ~0\%	& 1.3 \\ \hline
WNIL	& ~0\%	& 5.41 \\ \hline
DSWI	& 0.08\%	& 45 \\ \hline
\end{tabular}

\end{footnotesize}
\caption{Table showing error rate in picking the best traversal on dacapo dataset for each of the analysis and impact in execution time due to the error.}
\end{figure}


==> tex-figures/hand-optimized.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}
	\footnotesize
	\centering
	\caption{Overhead incurred by Hybrid approach when compared with hand optimized analysis using decision tree (\fignref{fig:decision-diagram}) as guideline.}
	\setlength{\tabcolsep}{2pt}
	\begin{tabular}{cr}
		\toprule
		Analysis & Increase in Runtime \\
		\midrule
		CP, CSD, LIC, DOM, PDOM, RD & 1\% \\
		DC, USA, VFR, MWN, AE, LMA, LMNA, LV, NA, RS, VBE, SS, UDV, UIR, WNIL  & 2\% \\
		\bottomrule
	\end{tabular}%
	\label{tab:hand-optimize-table}%
\end{table}%

==> tex-figures/loop-precision.tex <==
\begin{figure}[h]
\centering
\subfloat[CP]{
\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-cp.png}}
\label{fig:loop-cp}
}
\subfloat[CSD]{
\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-csd.png}}
\label{fig:loop-csd}
}
\subfloat[DC]{
\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-dc.png}}
\label{fig:loop-dc}
}
\subfloat[LIC]{
\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-lic.png}}
\label{fig:loop-lic}
}\\
\subfloat[USA]{
\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-usa.png}}
\label{fig:loop-use}
}
\subfloat[VFR]{
	\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-vfr.png}}
	\label{fig:loop-vfr}
}
\subfloat[MWN]{
	\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-mwn.png}}
	\label{fig:loop-mwn}
}
\subfloat[AE]{
\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-ae.png}}
\label{fig:loop-ae}
}\\
\subfloat[LMA]{
\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-lma.png}}
\label{fig:loop-lma}
}
\subfloat[LMNA]{
\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-lmna.png}}
\label{fig:loop-lmna}
}
\subfloat[LV]{
\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-lv.png}}
\label{fig:loop-lv}
}
\subfloat[NA]{
\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-na.png}}
\label{fig:loop-na}
}\\
\subfloat[RD]{
\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-rd.png}}
\label{fig:loop-rd}
}
\subfloat[RS]{
\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-rs.png}}
\label{fig:loop-rs}
}
\subfloat[VBE]{
\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-vbe.png}}
\label{fig:loop-vbe}
}
\subfloat[SS]{
	\fbox{\includegraphics[width=0.22\linewidth]{figures/loop-ss.png}}
	\label{fig:loop-ss}
}\\
\caption{Scatter charts for analyses that have loop sensitive traversals. 
%$x$-axis lists the CFGs in the increasing of the node size. 
On $y$-axis, 1 indicates a correct traversal strategy prediction and 0 indicates 
a mis-prediction.}
\label{fig:loops}
\end{figure}



==> tex-figures/misprediction-graph.tex <==
\begin{figure}[h]
\centering

\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/cp-crop.pdf}
\label{fig:mis-cp}
\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/csd-crop.pdf}
\label{fig:mis-csd}
\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/DC-crop.pdf}
\label{fig:mis-dc}
\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/LIC-crop.pdf}
\label{fig:mis-lic}
\\
\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/usa-crop.pdf}
\label{fig:mis-use}
	\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/vfr-crop.pdf}
	\label{fig:mis-vfr}
	\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/mwn-crop.pdf}
	\label{fig:mis-mwn}
\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/AE-crop.pdf}
\label{fig:mis-ae}
\\
\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/LMA-crop.pdf}
\label{fig:mis-lma}
\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/LMNA-crop.pdf}
\label{fig:mis-lmna}
\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/LV-crop.pdf}
\label{fig:mis-lv}
\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/NA-crop.pdf}
\label{fig:mis-na}
\\
\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/rd-crop.pdf}
\label{fig:mis-rd}
\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/rs-crop.pdf}
\label{fig:mis-rs}
\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/VBE-crop.pdf}
\label{fig:mis-vbe}
	\includegraphics[width=0.22\linewidth]{tex-figures/misprediction/SS-crop.pdf}
	\label{fig:mis-ss}
\\
\caption{Hybrid approach's performance against best approaches for mis-predicted graphs.}
\label{fig:mis-graph}
\end{figure}



==> tex-figures/paths-table.tex <==
\begin{figure}
	\centering
	\scriptsize
	\resizebox{1.0\linewidth}{!}{
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lrrrrrrrrrrr}
\toprule
      & P1    & P2    & P3    & P4    & P5    & P6    & P7    & P8    & P9    & P10   & P11 \\
\midrule
CP    & \cellcolor{lightgreen}35\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}50\% \\
CSD   & \cellcolor{lightgreen}35\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}50\% \\
DC    & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}35\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightgreen}50\% \\
LIC   & \cellcolor{lightgreen}35\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}50\% \\
USA   & \cellcolor{lightgreen}35\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}50\% \\
VFR   & \cellcolor{lightgreen}35\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}50\% \\
MWN   & \cellcolor{lightgreen}35\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}50\% \\
AE    & \cellcolor{lightgreen}69\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}21\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
DOM   & \cellcolor{lightgreen}69\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}21\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}7\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}3\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
LMA   & \cellcolor{lightgreen}69\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}21\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
LMNA  & \cellcolor{lightgreen}69\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}21\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
LV    & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}69\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}21\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\% \\
NA    & \cellcolor{lightgreen}69\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}21\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
PDOM  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}69\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}21\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}7\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}3\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
RD    & \cellcolor{lightgreen}69\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}21\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
RS    & \cellcolor{lightgreen}69\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}21\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
VBE   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}69\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}21\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\% \\
SS    & \cellcolor{lightgreen}69\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}21\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
UDV   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}100\% \\
UIR   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}100\% \\
WNIL  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}100\% \\
\midrule
Overall & \cellcolor{lightgreen}34.54\%   & \cellcolor{lightgreen}9.87\%   & \cellcolor{lightblack}10.32\%   & \cellcolor{lightblack}2.95\%   & \cellcolor{lightblue}0.26\%   & \cellcolor{lightblue}0.26\%   & \cellcolor{lightblue}0.11\%   & \cellcolor{lightblue}0.11\%   & \cellcolor{lightblack}4.78\%   & \cellcolor{lightblack}1.10\%   & \cellcolor{lightgreen}35.71\% \\
\bottomrule
\end{tabular}%
}
	\caption{Distribution of decisions over the paths of the decision tree. 
	\footnotesize Background colors indicate ranges of values: \colorbox{lightred}{0\%}, 
	\colorbox{lightblue}{(0\%, 1\%)}, \colorbox{lightblack}{[1\%, 10\%)} and \colorbox{lightgreen}{[10\%, 100\%]}.}

	\label{fig:decision-distribution}
	\label{fig:paths-sf}
\end{figure}

%\begin{table}%
%\centering
%\scriptsize
%\caption{Reduction in running times. Background colors indicate the ranges of 
%values: \colorbox{lightred}{0\%}, \colorbox{lightblue}{(0\%, 1\%)}, 
%\colorbox{lightblack}{[1\%, 10\%)} and \colorbox{lightgreen}{[10\%, 100\%]}.}
%\begin{tabular}{lrrrrrrrrrrr}
%\toprule
      %& P1    & P2    & P3    & P4    & P5    & P6    & P7    & P8    & P9    & P10   & P11 \\
%\midrule
%CP    & 32\%  & 0\%   & 13\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 5\%   & 0\%   & 50\% \\
%CSD   & 32\%  & 0\%   & 13\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 5\%   & 0\%   & 50\% \\
%DC    & 0\%   & 32\%  & 0\%   & 13\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 5\%   & 50\% \\
%USA   & 22\%  & 0\%   & 8\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 3\%   & 0\%   & 67\% \\
%AE    & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\%   & 0\% \\
%Dom   & 65\%  & 0\%   & 25\%  & 0\%   & 7\%   & 0\%   & 2\%   & 0\%   & 0\%   & 0\%   & 0\% \\
%LIC   & 22\%  & 0\%   & 8\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 3\%   & 0\%   & 67\% \\
%LMA   & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\%   & 0\% \\
%LMNA  & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\%   & 0\% \\
%LV    & 0\%   & 2\%   & 0\%   & 97\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\% \\
%NA    & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\%   & 0\% \\
%PDOM  & 0\%   & 65\%  & 0\%   & 25\%  & 0\%   & 7\%   & 0\%   & 2\%   & 0\%   & 0\%   & 0\% \\
%RD    & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\%   & 0\% \\
%RS    & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\%   & 0\% \\
%VBE   & 0\%   & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\% \\
%UDV   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 100\% \\
%UIR   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 100\% \\
%WNIL  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 100\% \\
%\midrule
%Overall & 13.99\% & 5.09\% & 5.47\% & 53.01\% & 0.14\% & 0.14\% & 0.05\% & 0.05\% & 1.90\% & 0.57\% & 19.59\% \\
%\bottomrule
%\end{tabular}%
%\label{tab:decision-distribution}
%\end{table}

%\begin{figure}[!t]
	%\centering
	%\subfloat[DaCapo] {
		%\includegraphics[width=0.8\linewidth]{ecoop-figures/distribution-decision-dacapo.png}
		%\label{fig:paths-dacapo}
	%}\\
	%\subfloat[SourceForge] {
	%\includegraphics[width=0.8\linewidth]{ecoop-figures/distribution-decision-sf.png}
		%\label{fig:paths-sf}
	%}\\
	%\subfloat[All analyses] {
	%\includegraphics[width=0.8\linewidth]{ecoop-figures/distribution-decision-overall.png}
		%\label{fig:paths-all}
	%}
	%\caption{Distribution of decisions over the paths of the decision tree.}
	%\label{fig:decision-distribution}
%\end{figure}


==> tex-figures/paths-table2.tex <==
\begin{figure*}[h]
	\centering
	\scriptsize
	%\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrrrrrrrrrrr}
\toprule
      & P1    & P2    & P3    & P4    & P5    & P6    & P7    & P8    & P9    & P10   & P11 \\
\midrule
CP    & \cellcolor{lightgreen}32\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}13\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}\cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}50\% \\
CSD   & \cellcolor{lightgreen}32\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}13\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}50\% \\
DC    & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}32\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}13\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightgreen}50\% \\
LIC   & \cellcolor{lightgreen}32\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}13\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}50\% \\
USA   & \cellcolor{lightgreen}32\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}13\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}50\% \\
VFR   & \cellcolor{lightgreen}32\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}13\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}50\% \\
MWN   & \cellcolor{lightgreen}32\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}13\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}5\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}50\% \\
AE    & \cellcolor{lightgreen}65\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}25\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
DOM   & \cellcolor{lightgreen}65\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}25\%  & \cellcolor{lightred}0\%   & \cellcolor{lightblack}7\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}2\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
LMA   & \cellcolor{lightgreen}65\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}25\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
LMNA  & \cellcolor{lightgreen}65\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}25\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
LV   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}65\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}25\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%  & \cellcolor{lightred}0\% \\
NA    & \cellcolor{lightgreen}65\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}25\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
PDOM  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}65\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}25\%  & \cellcolor{lightred}0\%   & \cellcolor{lightblack}7\%   & \cellcolor{lightred}0\%   & \cellcolor{lightblack}2\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
RD    & \cellcolor{lightgreen}65\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}25\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
RS    & \cellcolor{lightgreen}65\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}25\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
VBE   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}65\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}25\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%  & \cellcolor{lightred}0\% \\
SS    & \cellcolor{lightgreen}65\%  & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}25\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}10\%  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\% \\
UDV   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}100\% \\
UIR   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}100\% \\
WNIL  & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightred}0\%   & \cellcolor{lightgreen}100\% \\
\midrule
Overall & \cellcolor{lightgreen}32.46\% & \cellcolor{lightgreen}9.27\% & \cellcolor{lightgreen}12.69\% & \cellcolor{lightblack}3.62\% & \cellcolor{lightblue}0.26\% & \cellcolor{lightblue}0.26\% & \cellcolor{lightblue}0.10\% & \cellcolor{lightblue}0.10\% & \cellcolor{lightblack}4.50\% & \cellcolor{lightblack}1.04\% & \cellcolor{lightgreen}35.70\% \\
\bottomrule
\end{tabular}%
	\caption{Distribution of decisions over the paths of the decision tree for the DaCapo Dataset. 
	Background colors indicate the ranges of values: \colorbox{lightred}{0\%}, 
	\colorbox{lightblue}{(0\%, 1\%)}, \colorbox{lightblack}{[1\%, 10\%)} and \colorbox{lightgreen}{[10\%, 100\%]}.}
	\label{fig:paths-dacapo}
\end{figure*}

%\begin{table}%
%\centering
%\scriptsize
%\caption{Reduction in running times. Background colors indicate the ranges of 
%values: \colorbox{lightred}{0\%}, \colorbox{lightblue}{(0\%, 1\%)}, 
%\colorbox{lightblack}{[1\%, 10\%)} and \colorbox{lightgreen}{[10\%, 100\%]}.}
%\begin{tabular}{lrrrrrrrrrrr}
%\toprule
      %& P1    & P2    & P3    & P4    & P5    & P6    & P7    & P8    & P9    & P10   & P11 \\
%\midrule
%CP    & 32\%  & 0\%   & 13\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 5\%   & 0\%   & 50\% \\
%CSD   & 32\%  & 0\%   & 13\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 5\%   & 0\%   & 50\% \\
%DC    & 0\%   & 32\%  & 0\%   & 13\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 5\%   & 50\% \\
%USA   & 22\%  & 0\%   & 8\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 3\%   & 0\%   & 67\% \\
%AE    & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\%   & 0\% \\
%Dom   & 65\%  & 0\%   & 25\%  & 0\%   & 7\%   & 0\%   & 2\%   & 0\%   & 0\%   & 0\%   & 0\% \\
%LIC   & 22\%  & 0\%   & 8\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 3\%   & 0\%   & 67\% \\
%LMA   & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\%   & 0\% \\
%LMNA  & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\%   & 0\% \\
%LV    & 0\%   & 2\%   & 0\%   & 97\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\% \\
%NA    & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\%   & 0\% \\
%PDOM  & 0\%   & 65\%  & 0\%   & 25\%  & 0\%   & 7\%   & 0\%   & 2\%   & 0\%   & 0\%   & 0\% \\
%RD    & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\%   & 0\% \\
%RS    & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\%   & 0\% \\
%VBE   & 0\%   & 65\%  & 0\%   & 25\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 10\%  & 0\% \\
%UDV   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 100\% \\
%UIR   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 100\% \\
%WNIL  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 100\% \\
%\midrule
%Overall & 13.99\% & 5.09\% & 5.47\% & 53.01\% & 0.14\% & 0.14\% & 0.05\% & 0.05\% & 1.90\% & 0.57\% & 19.59\% \\
%\bottomrule
%\end{tabular}%
%\label{tab:decision-distribution}
%\end{table}

%\begin{figure}[!t]
	%\centering
	%\subfloat[DaCapo] {
		%\includegraphics[width=0.8\linewidth]{ecoop-figures/distribution-decision-dacapo.png}
		%\label{fig:paths-dacapo}
	%}\\
	%\subfloat[SourceForge] {
	%\includegraphics[width=0.8\linewidth]{ecoop-figures/distribution-decision-sf.png}
		%\label{fig:paths-sf}
	%}\\
	%\subfloat[All analyses] {
	%\includegraphics[width=0.8\linewidth]{ecoop-figures/distribution-decision-overall.png}
		%\label{fig:paths-all}
	%}
	%\caption{Distribution of decisions over the paths of the decision tree.}
	%\label{fig:decision-distribution}
%\end{figure}


==> tex-figures/precondition-result.tex <==
\newcommand{\receiver}{rcv}
\newcommand{\argument}{arg}

\begin{wrapfigure}[10]{l}{.54\columnwidth}
%\begin{figure}[t]%
\centering
\scriptsize
\setlength{\tabcolsep}{5.2pt}
\begin{tabular}{lrrr}
\toprule
Method & First & Second \\
\midrule
%equals(Object) & {\receiver} != null & {\argument} != null \\
split(String) & {\receiver} != null & !{\receiver}.isEmpty() \\
charAt(int) & {\receiver} != null & {\argument} < {\receiver}.length() \\
substring(int) & {\receiver} != null & {\argument} != -1 \\
\bottomrule
\end{tabular}%
\caption{Case study APM:~An excerpt of mined~preconditions.}
%{First and second most occurring preconditions for top-4 most frequently used methods in \lstinline|java.lang.String|.}
\label{fig:precondition-result}
%\end{figure}
\end{wrapfigure}

==> tex-figures/reduction-table-oopsla-guideline.tex <==
\begin{wrapfigure}{l}{.2\textwidth}
%\begin{figure}%
\centering
\scriptsize
\begin{tabular}{lrrrrrr|rrrrrr}
\toprule
\multicolumn{1}{l}{Analysis} & \multicolumn{1}{c|}{DaCapo}                    & \multicolumn{1}{c}{GitHub} \\
\midrule
\multicolumn{1}{l}{CP} & \cellcolor{lightblue}9\%  & \cellcolor{lightblue}5\%  \\
\multicolumn{1}{l}{CSD} & \cellcolor{lightblue}4\%  & \cellcolor{lightblack}12\% \\
\multicolumn{1}{l}{DC} & \cellcolor{lightblue}7\%  & \cellcolor{lightblue}7\%  \\
\multicolumn{1}{l}{LIC} & \cellcolor{lightblue}7\%  & \cellcolor{lightblack}19\% \\
\multicolumn{1}{l}{USA} & \cellcolor{lightblue}9\%  & \cellcolor{lightblue}9\% \\
\multicolumn{1}{l}{VFR} & \cellcolor{lightblack}15\%  & \cellcolor{lightblue}9\% \\
\multicolumn{1}{l}{MWN} & \cellcolor{lightblack}15\%  & \cellcolor{lightblue}9\% \\
\multicolumn{1}{l}{AE} & \cellcolor{lightblack}14\%  &  \cellcolor{lightblack}11\% \\
\multicolumn{1}{l}{DOM} & \cellcolor{lightblue}6\%  & \cellcolor{lightblue}6\% \\
\multicolumn{1}{l}{LMA} & \cellcolor{lightblue}6\%  & \cellcolor{lightblue}6\% \\
\multicolumn{1}{l}{LMNA} & \cellcolor{lightblue}9\%  & \cellcolor{lightblue}7\% \\
\multicolumn{1}{l}{LV} & \cellcolor{lightblack}11\%  & \cellcolor{lightblack}11\%  \\
\multicolumn{1}{l}{NA} & \cellcolor{lightblack}10\%  & \cellcolor{lightblack}10\%  \\
\multicolumn{1}{l}{PDOM} & \cellcolor{lightblack}10\%  & \cellcolor{lightblack}24\% \\
\multicolumn{1}{l}{RD} & \cellcolor{lightblue}9\%  & \cellcolor{lightblue}5\% \\
\multicolumn{1}{l}{RS} & \cellcolor{lightblack}28\%  & \cellcolor{lightblue}7\% \\
\multicolumn{1}{l}{VBE} & \cellcolor{lightblack}13\%  & \cellcolor{lightblack}10\% \\
\multicolumn{1}{l}{SS} & \cellcolor{lightblack}22\%  & \cellcolor{lightblack}10\%  \\
\multicolumn{1}{l}{UDV} &  \cellcolor{lightblue}3\%   &  \cellcolor{lightblue}0\%  \\
\multicolumn{1}{l}{UIR} &  \cellcolor{lightblue}0\%   &  \cellcolor{lightblue}0\%  \\
\multicolumn{1}{l}{WNIL} &  \cellcolor{lightblue}2\%   &  \cellcolor{lightblue}0\% \\
\bottomrule
\end{tabular}%
\caption{Reduction in running times against hand optimized analysis. Background colors indicate the ranges of 
values: \colorbox{lightred}{no reduction}, \colorbox{lightblue}{(0\%, 10\%)}, 
\colorbox{lightblack}{[10\%, 50\%)} and \colorbox{lightgreen}{[50\%, 100\%]}.}
\label{fig:reduction-oopsla}
%\end{figure}
\end{wrapfigure}


==> tex-figures/reduction-table2.tex <==
\begin{table}[ht!]
\caption{Reduction in running times. \footnotesize Background colors indicate ranges of 
values: \colorbox{lightred}{no reduction}, \colorbox{lightblue}{(0\%, 10\%)}, 
\colorbox{lightblack}{[10\%, 50\%)} and \colorbox{lightgreen}{[50\%, 100\%]}.}
\label{tab:reduction-analyses-short}
\centering
\scriptsize
%\subfloat[Time reduction for each analysis.] {
%\resizebox{1.0\linewidth}{!}{
\setlength{\tabcolsep}{1.8pt}
\begin{tabular}{lrrrrrr||lrrrrrr}
\toprule
\multicolumn{1}{l}{Analysis} & DFS   & PO    & RPO   & WPO   & WRPO  & ANY    & \multicolumn{1}{l}{Analysis} & DFS   & PO    & RPO   & WPO   & WRPO  & ANY    \\
\midrule
\multicolumn{1}{l}{CP} & \cellcolor{lightblack}17\%  & \cellcolor{lightgreen}83\%  &  \cellcolor{lightblue}9\%   & \cellcolor{lightgreen}66\%  &  \cellcolor{lightblack}11\%   & \cellcolor{lightgreen}72\%  & \multicolumn{1}{l}{LV} & \cellcolor{lightblack}38\%  & \cellcolor{lightblack}30\%  & \cellcolor{lightgreen}84\%  &  \cellcolor{lightblack}11\%   & \cellcolor{lightblack}56\%  & \cellcolor{lightgreen}75\%  \\
\multicolumn{1}{l}{CSD} & \cellcolor{lightblack}41\%  & \cellcolor{lightgreen}93\%  & \cellcolor{lightblack}39\%  & \cellcolor{lightgreen}74\%  &  \cellcolor{lightblue}4\%   & \cellcolor{lightgreen}89\%  & \multicolumn{1}{l}{NA} & \cellcolor{lightblack}26\%  & \cellcolor{lightgreen}88\%  & \cellcolor{lightblack}30\%  & \cellcolor{lightblack}50\%  &  \cellcolor{lightblue}10\%   & \cellcolor{lightgreen}80\%  \\
\multicolumn{1}{l}{DC} & \cellcolor{lightblack}41\%  & \cellcolor{lightblack}30\%  & \cellcolor{lightgreen}89\%  &  \cellcolor{lightblue}7\%   & \cellcolor{lightgreen}64\%  & \cellcolor{lightgreen}81\%  & \multicolumn{1}{l}{PDOM} & \cellcolor{lightblack}51\%  & \cellcolor{lightblack}41\%  & \cellcolor{lightgreen}95\%  &  \cellcolor{lightblue}10\%   & \cellcolor{lightgreen}72\%  & \cellcolor{lightgreen}95\%  \\
\multicolumn{1}{l}{LIC} & \cellcolor{lightblack}17\%  & \cellcolor{lightgreen}84\%  &  \cellcolor{lightblue}8\%   & \cellcolor{lightgreen}67\%  &  \cellcolor{lightblue}7\%   & \cellcolor{lightgreen}73\%  & \multicolumn{1}{l}{RD} & \cellcolor{lightblack}15\%  & \cellcolor{lightgreen}80\%  &  \cellcolor{lightblue}7\%   & \cellcolor{lightgreen}62\%  &  \cellcolor{lightblue}9\%   & \cellcolor{lightgreen}68\%  \\
\multicolumn{1}{l}{USA} & \cellcolor{lightblack}36\%  & \cellcolor{lightgreen}92\%  & \cellcolor{lightblack}34\%  & \cellcolor{lightgreen}72\%  &  \cellcolor{lightblue}9\%   & \cellcolor{lightgreen}87\%  & \multicolumn{1}{l}{RS} & \cellcolor{lightblack}31\%  & \cellcolor{lightblack}31\%  & \cellcolor{lightblack}30\%  & \cellcolor{lightblack}31\%  & \cellcolor{lightblack}28\%  & \cellcolor{lightblack}30\%  \\
\multicolumn{1}{l}{VFR} & \cellcolor{lightblack}20\%  & \cellcolor{lightblack}41\%  & \cellcolor{lightblack}18\%  & \cellcolor{lightgreen}51\%  & \cellcolor{lightblack}15\%  & \cellcolor{lightgreen}62\%  & \multicolumn{1}{l}{VBE} & \cellcolor{lightblack}40\%  & \cellcolor{lightblack}36\%  & \cellcolor{lightgreen}88\%  &  \cellcolor{lightblack}13\%   & \cellcolor{lightgreen}76\%  & \cellcolor{lightgreen}81\%  \\
\multicolumn{1}{l}{MWN} & \cellcolor{lightblack}21\%  & \cellcolor{lightblack}35\%  & \cellcolor{lightblack}16\%  & \cellcolor{lightblack}35\%  & \cellcolor{lightblack}22\%  & \cellcolor{lightblack}49\%  & \multicolumn{1}{l}{SS} & \cellcolor{lightblack}26\%  & \cellcolor{lightblack}39\%  & \cellcolor{lightblack}22\%  & \cellcolor{lightblack}37\%  & \cellcolor{lightblack}25\%  & \cellcolor{lightgreen}57\%  \\
\multicolumn{1}{l}{AE} & \cellcolor{lightblack}40\%  &  \cellcolor{lightblack}14\%   & \cellcolor{lightblack}39\%  & \cellcolor{lightgreen}73\%  &  \cellcolor{lightblack}14\%   & \cellcolor{lightgreen}87\%  & \multicolumn{1}{l}{UDV} &  \cellcolor{lightblue}6\%   &  \cellcolor{lightblue}5\%   &  \cellcolor{lightblue}6\%   &  \cellcolor{lightblue}10\%   &  \cellcolor{lightblue}9\%   &  \cellcolor{lightblue}3\%  \\
\multicolumn{1}{l}{DOM} & \cellcolor{lightblack}54\%  & \cellcolor{lightgreen}97\%  & \cellcolor{lightblack}48\%  & \cellcolor{lightgreen}70\%  &  \cellcolor{lightblue}6\%   & \cellcolor{lightgreen}95\%  & \multicolumn{1}{l}{UIR} &  \cellcolor{lightblue}2\%   &  \cellcolor{lightblue}2\%   &  \cellcolor{lightblue}1\%   & \cellcolor{lightblue}3\%   & \cellcolor{lightblue}3\%   & \cellcolor{lightblue}0\%   \\
\multicolumn{1}{l}{LMA} & \cellcolor{lightblack}35\%  & \cellcolor{lightblack}46\%  & \cellcolor{lightblack}28\%  & \cellcolor{lightgreen}74\%  &  \cellcolor{lightblue}6\%   & \cellcolor{lightblack}46\%  & \multicolumn{1}{l}{WNIL} &  \cellcolor{lightblue}3\%   &  \cellcolor{lightblue}4\%   &  \cellcolor{lightblue}5\%   &  \cellcolor{lightblue}6\%   &  \cellcolor{lightblue}8\%   & \cellcolor{lightblue}2\%  \\
\cline{8-14}
\multicolumn{1}{l}{LMNA} & \cellcolor{lightblack}29\%  & \cellcolor{lightblack}39\%  & \cellcolor{lightblack}22\%  & \cellcolor{lightgreen}68\%  &  \cellcolor{lightblue}9\%   & \cellcolor{lightblack}41\%  & \multicolumn{1}{l}{Overall} &  \cellcolor{lightblack}31\%   &  \cellcolor{lightgreen}83\%   &  \cellcolor{lightgreen}70\%   &  \cellcolor{lightblack}55\%   &  \cellcolor{lightblack}35\%   &  \cellcolor{lightgreen}81\%  \\
%\midrule
%\multicolumn{1}{l}{Overall} &  \cellcolor{lightblack}31\%   &  \cellcolor{lightgreen}83\%   &  \cellcolor{lightgreen}70\%   &  \cellcolor{lightblack}55\%   &  \cellcolor{lightblack}35\%   &  \cellcolor{lightgreen}81\%  \\
\bottomrule
\end{tabular}%

%\begin{tabular}{lrrrrrr}
%\toprule
%\multicolumn{1}{l}{Overall} &  \cellcolor{lightblack}31\%   &  \cellcolor{lightgreen}83\%   &  \cellcolor{lightgreen}70\%   &  \cellcolor{lightblack}55\%   &  \cellcolor{lightblack}35\%   &  \cellcolor{lightgreen}81\%  \\
%\bottomrule
%\end{tabular}%
\end{table}


==> tex-figures/significance_table.tex <==

\begin{figure}[t]
\begin{footnotesize}
\setlength{\tabcolsep}{0.5pt}
\begin{tabular}{ | c |>{\columncolor[gray]{0.8}} c |>{\columncolor[gray]{0.8}} c |>{\columncolor[gray]{0.8}} c |>{\columncolor{SkyBlue}} c |>{\columncolor{SkyBlue}} c |>{\columncolor{SkyBlue}} c |>{\columncolor{Salmon}} c |>{\columncolor{Salmon}} c |>{\columncolor{Salmon}} c | }
\hline
	\multirow{1}{*}{\textbf{Analysis}} & \multicolumn{3}{ c|}{Node size < 300}  & \multicolumn{3}{ c|}{Node size - 300 to 500} & \multicolumn{3}{ c|}{Node size > 500}  \\ \hhline{|*1{>{\arrayrulecolor{white}} }*{10}{>{\arrayrulecolor{black}}-}|}
	 & DFS & RPO/PO & Worklist & DFS & RPO/PO & Worklist & DFS & RPO/PO & Worklist \\ \hline
	\cellcolor{LimeGreen} DOM & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark &  \checkmark & \checkmark & \checkmark & = \\ \hline
	\cellcolor{LimeGreen}PDOM & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark & = & \checkmark & \checkmark & = \\ \hline
	\cellcolor{LimeGreen}LV & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark & = & \checkmark & \checkmark & = \\ \hline
	\cellcolor{LimeGreen}RD & \checkmark & \checkmark & \checkmark & $\times$ & $\times$ & = & $\times$ & $\times$ & = \\ \hline
	\cellcolor{LimeGreen}LMA & \checkmark & \checkmark & \checkmark & $\times$ & $\times$ & = & $\times$ & $\times$ & = \\ \hline
	\cellcolor{LimeGreen}LMNA & \checkmark & \checkmark & \checkmark &  \checkmark & \checkmark & = & $\times$ & $\times$ & = \\ \hline
	\cellcolor{LimeGreen}AE & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark & = & \checkmark & \checkmark & = \\ \hline
	\cellcolor{LimeGreen}VBE & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark & = & \checkmark & \checkmark & = \\ \hline
	\cellcolor{LimeGreen}USA & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark & = & \checkmark & \checkmark & = \\ \hline
	\cellcolor{LimeGreen}RS & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark & = & \checkmark & \checkmark & = \\ \hline
	\cellcolor{LimeGreen}NA & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark & = & \checkmark & \checkmark & = \\ \hline
	\cellcolor{LimeGreen}CSD & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark & = & \checkmark & \checkmark & = \\ \hline
	\cellcolor{LimeGreen}LIC & \checkmark & \checkmark & \checkmark & $\times$ & $\times$ & = & $\times$ & $\times$ & = \\ \hline
	\cellcolor{LimeGreen}DC & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark & = & \checkmark & \checkmark & = \\ \hline
	\cellcolor{LimeGreen}CP & \checkmark & \checkmark & \checkmark & $\times$ & $\times$ & = & $\times$ & $\times$ & = \\ \hline
	\cellcolor{Peach}WNIL & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark & = & \checkmark & \checkmark & = \\ \hline
	\cellcolor{Peach}DEI & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark &  \checkmark & \checkmark & \checkmark & \checkmark \\ \hline
	\cellcolor{Peach}IL & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark &  \checkmark & \checkmark & \checkmark & \checkmark \\ \hline
	\cellcolor{Peach}UIR & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark &  \checkmark & \checkmark & \checkmark & \checkmark \\ \hline
	\cellcolor{Peach}UDV & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark &  \checkmark & \checkmark & \checkmark & \checkmark \\ \hline
\end{tabular}

\hfill \break \break  \hspace{3ex}
\begin{tabular}{ |c|c| } 
 \hline
 \cellcolor{SkyBlue} Data flow analysis & \cellcolor{Salmon} Data flow in-sensitive analysis \\
 \hline
\end{tabular}




\end{footnotesize}
\caption{Table showing significance test result for nodes of differnt sizes.
The tick symbol indicates significant gain and the cross symbol indiactes
insignificant gain. Equals symbol indicates that we do get gain compared to the approach but is not significant enough.}
\end{figure}


==> tex-figures/time-breakdown-table-v1.tex <==
%\begin{table}[t]
	%\centering
	%\scriptsize
	%\caption{Time contribution of each phase (in miliseconds).}
	%\setlength{\tabcolsep}{5pt}
%\begin{tabular}{rrccrr}
%\toprule
%\multicolumn{1}{l}{Analysis} & Static & \multicolumn{2}{c}{CFG creation} & \multicolumn{2}{c}{Traversal} \\
%\cmidrule(lr){3-4} \cmidrule(lr){5-6}
%\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & Avg.  & Total & \multicolumn{1}{c}{Avg.} & \multicolumn{1}{c}{Total} \\
%\midrule
%\multicolumn{1}{l}{CP} &         53  & \multirow{18}{*}{0.05} & \multirow{18}{*}{13,170} &           0.17  &    49,297  \\
%\multicolumn{1}{l}{CSD} &         60  &       &       &           0.15  &    43,670  \\
%\multicolumn{1}{l}{DC} &         45  &       &       &           0.15  &    41,651  \\
%\multicolumn{1}{l}{LIC} &         69  &       &       &           0.16  &    47,122  \\
%\multicolumn{1}{l}{USA} &         90  &       &       &           0.14  &    41,168  \\
%\multicolumn{1}{l}{AE} &         43  &       &       &           0.14  &    40,190  \\
%\multicolumn{1}{l}{DOM} &         35  &       &       &           0.17  &    49,316  \\
%\multicolumn{1}{l}{LMA} &         76  &       &       &           0.14  &    39,382 \\
%\multicolumn{1}{l}{LMNA} &         80  &       &       &           0.14  &    40,081  \\
%\multicolumn{1}{l}{LV} &         32  &       &       &           0.13  &    36,130  \\
%\multicolumn{1}{l}{NA} &         64  &       &       &           0.12  &    33,488  \\
%\multicolumn{1}{l}{PDOM} &         34  &       &       &           0.15  &    44,103  \\
%\multicolumn{1}{l}{RD} &         48  &       &       &           0.15  &    44,259  \\
%\multicolumn{1}{l}{RS} &         28  &       &       &           0.12  &    33,267  \\
%\multicolumn{1}{l}{VBE} &         44  &       &       &           0.13  &    36,037  \\
%\multicolumn{1}{l}{UDV} &         10  &       &       &           0.10  &    28,517  \\
%\multicolumn{1}{l}{UIR} &         14  &       &       &           0.10  &    28,046  \\
%\multicolumn{1}{l}{WNIL} &         15  &       &       &           0.10  &    28,708  \\
%\bottomrule
%\end{tabular}%
	%\label{tab:time-break-down-table}%
%\end{table}%

\begin{table}[t]
	\centering
	\scriptsize
	\caption{Time contribution of each phase (in miliseconds).}
	%\setlength{\tabcolsep}{5pt}
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{rrccrrrccrr}
\toprule
\multicolumn{1}{c}{Analysis} & \multicolumn{5}{c}{DaCapo}            & \multicolumn{5}{c}{SourceForge} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{Static} & \multicolumn{2}{c}{CFG creation} & \multicolumn{2}{c}{Traversal} & \multicolumn{1}{c}{Static} & \multicolumn{2}{c}{CFG creation} & \multicolumn{2}{c}{Traversal} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & Avg.  & Total & \multicolumn{1}{c}{Avg.} & \multicolumn{1}{c}{Total} & \multicolumn{1}{c}{} & Avg.  & Total & \multicolumn{1}{c}{Avg.} & \multicolumn{1}{c}{Total} \\
\midrule
\multicolumn{1}{l}{CP} &          53  & \multirow{18}{*}{0.05} & \multirow{18}{*}{13,171} &    0.17  &          49,298  &               53  & \multirow{18}{*}{0.08} & \multirow{18}{*}{13,576K} &           0.45  &      72,971K  \\
\multicolumn{1}{l}{CSD} &          60  &       &       &    0.15  &          43,671  &               60  &       &       &           0.46  &      74,656K  \\
\multicolumn{1}{l}{DC} &          45  &       &       &    0.15  &          41,651  &               45  &       &       &           0.43  &      70,898K  \\
\multicolumn{1}{l}{LIC} &          69  &       &       &    0.16  &          47,123  &               69  &       &       &           0.42  &      68,755K  \\
\multicolumn{1}{l}{USA} &          90  &       &       &    0.14  &          41,168  &               90  &       &       &           0.37  &      72,042K  \\
\multicolumn{1}{l}{AE} &          43  &       &       &    0.14  &          40,190  &               43  &       &       &           0.45  &      73,412K  \\
\multicolumn{1}{l}{DOM} &          35  &       &       &    0.17  &          49,316  &               35  &       &       &           0.44  &      71,810K  \\
\multicolumn{1}{l}{LMA} &          76  &       &       &    0.14  &          39,383  &               76  &       &       &           0.37  &      60,055K  \\
\multicolumn{1}{l}{LMNA} &          80  &       &       &    0.14  &          40,082  &               80  &       &       &           0.37  &      60,064K  \\
\multicolumn{1}{l}{LV} &          32  &       &       &    0.13  &          36,131  &               32  &       &       &           0.33  &      54,172K  \\
\multicolumn{1}{l}{NA} &          64  &       &       &    0.12  &          33,489  &               64  &       &       &           0.41  &      66,361K  \\
\multicolumn{1}{l}{PDOM} &          34  &       &       &    0.15  &          44,103  &               34  &       &       &           0.43  &      70,825K  \\
\multicolumn{1}{l}{RD} &          48  &       &       &    0.15  &          44,259  &               48  &       &       &           0.37  &      59,989K  \\
\multicolumn{1}{l}{RS} &          28  &       &       &    0.12  &          33,267  &               28  &       &       &           0.38  &      61,587K  \\
\multicolumn{1}{l}{VBE} &          44  &       &       &    0.13  &          36,038  &               44  &       &       &           0.41  &      66,344K  \\
\multicolumn{1}{l}{UDV} &          10  &       &       &    0.10  &          28,517  &               10  &       &       &           0.37  &      59,707K  \\
\multicolumn{1}{l}{UIR} &          14  &       &       &    0.10  &          28,046  &               14  &       &       &           0.35  &      57,631K  \\
\multicolumn{1}{l}{WNIL} &          15  &       &       &    0.10  &          28,708  &               15  &       &       &           0.37  &      60,333K  \\
\bottomrule
\end{tabular}%

	\label{tab:time-break-down-table}%
\end{table}%


==> tex-helpers/macros.tex <==
% $Id: macros.tex,v 1.9 2013/02/19 07:02:00 rdyer Exp $

\usepackage{balance}
\usepackage{relsize}
\usepackage[T1]{fontenc}
\usepackage{times}
\usepackage{url}
\usepackage{amssymb}
\usepackage{amsmath}
%\usepackage{cite}
\usepackage{fancyvrb}
\usepackage{colortbl}
\usepackage[dvipsnames]{xcolor}
\usepackage{xspace}
\usepackage{comment}

\usepackage{hhline}

% Command for figures
\usepackage{epsfig}
\usepackage{subfigure}
\usepackage{multirow}
\graphicspath{{figures/}}
\usepackage{graphicx}

% Added listing for code listings
\usepackage{listings}

% Packages for algorithms
\usepackage{algorithm}
\usepackage{algorithmic}



% *** MISC UTILITY PACKAGES ***
%
%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%   % dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/tex-archive/macros/latex/contrib/oberdiek/
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.




% *** FLOAT PACKAGES ***
%
%\usepackage{fixltx2e}
% fixltx2e, the successor to the earlier fix2col.sty, was written by
% Frank Mittelbach and David Carlisle. This package corrects a few problems
% in the LaTeX2e kernel, the most notable of which is that in current
% LaTeX2e releases, the ordering of single and double column floats is not
% guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
% single column figure to be placed prior to an earlier double column
% figure. The latest version and documentation can be found at:
% http://www.ctan.org/tex-archive/macros/latex/base/



%\usepackage{stfloats}
% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% the ability to do double column floats at the bottom of the page as well
% as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% LaTeX2e). It also provides a command:
%\fnbelowfloat
% to enable the placement of footnotes below bottom floats (the standard
% LaTeX2e kernel puts them above bottom floats). This is an invasive package
% which rewrites many portions of the LaTeX2e float routines. It may not work
% with other packages that modify the LaTeX2e float routines. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/tex-archive/macros/latex/contrib/sttools/
% Documentation is contained in the stfloats.sty comments as well as in the
% presfull.pdf file. Do not use the stfloats baselinefloat ability as IEEE
% does not allow \baselineskip to stretch. Authors submitting work to the
% IEEE should note that IEEE rarely uses double column equations and
% that authors should try to avoid such use. Do not be tempted to use the
% cuted.sty or midfloat.sty packages (also by Sigitas Tolusis) as IEEE does
% not format its papers in such ways.



% Help LaTeX not violate the column margins
\tolerance=50000


% settings for listings
\definecolor{lightgray}{gray}{0.97}
\definecolor{darkgray}{gray}{0.5}
\definecolor{OliveGreen}{cmyk}{0.64,0,0.95,0.40}

\lstset{
	language=bash, emph={},
	mathescape=false, escapechar=@,
	backgroundcolor=\color{lightgray},
	commentstyle=\color{darkgray},
	keywordstyle=\color{OliveGreen}\bfseries,
	basicstyle=\scriptsize\sffamily,
	numberstyle=\scriptsize\sffamily,
	emphstyle=\bfseries,
	numbers=left, stepnumber=1,
	numberblanklines=false,
	numberstyle=\tiny,
	numbersep=-3pt,
	frame=none, framexleftmargin=0pt, framexrightmargin=0pt, 
	%xleftmargin=15pt, xrightmargin=4pt,
	columns=flexible, breaklines=true,
	showspaces=false, showstringspaces=false, showtabs=false, tabsize=2,
	morekeywords={output, foreach, exists, ifsome, of}
}


% cross referencing
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\fignref}[1]{Figure~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\secnref}[1]{Section~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}

\newcommand{\etal}{~\textit{et al.}\@\xspace}
\newcommand{\lang}{\textit{Boa}\xspace}

% Allow figures to take up the entire page
\renewcommand\floatpagefraction{.99}
\renewcommand\topfraction{.99}
\renewcommand\bottomfraction{.90}
\renewcommand\textfraction{.01}

% avoid orphans and widows
\clubpenalty = 10000
\widowpenalty = 10000
\displaywidowpenalty = 10000


